Artificial diffusion for convective and acoustic low Mach number flows II: Application to Liou-Steffen, Zha-Bilgen and Toro-Vasquez convection-pressure flux splittings

Liou-Steffen splitting (AUSM) schemes are popular for low Mach number simulations, however, like many numerical schemes for compressible flow they require careful modification to accurately resolve convective features in this regime. Previous analyses of these schemes usually focus only on a single discrete scheme at the convective limit, only considering flow with acoustic effects empirically, if at all. In our recent paper Hope-Collins & di Mare, 2023 we derived constraints on the artificial diffusion scaling of low Mach number schemes for flows both with and without acoustic effects, and applied this analysis to Roe-type finite-volume schemes. In this paper we form approximate diffusion matrices for the Liou-Steffen splitting, as well as the closely related Zha-Bilgen and Toro-Vasquez splittings. We use the constraints found in Hope-Collins & di Mare, 2023 to derive and analyse the required scaling of each splitting at low Mach number. By transforming the diffusion matrices to the entropy variables we can identify erroneous diffusion terms compared to the ideal form used in Hope-Collins & di Mare, 2023. These terms vanish asymptotically for the Liou-Steffen splitting, but result in spurious entropy generation for the Zha-Bilgen and Toro-Vasquez splittings unless a particular form of the interface pressure is used. Numerical examples for acoustic and convective flow verify the results of the analysis, and show the importance of considering the resolution of the entropy field when assessing schemes of this type.

==> abstract1.tex <==
%TC:ignore
\noindent \textbf{Paper I: Analysis of the modified equations, and application to Roe-type schemes}
%TC:endignore

\noindent Three asymptotic limits exist for the Euler equations at low Mach number - purely convective, purely acoustic, and mixed convective-acoustic.
Standard collocated density-based numerical schemes for compressible flow are known to fail at low Mach number due to the incorrect asymptotic scaling of the artificial diffusion.
Previous studies of this class of schemes have shown a variety of behaviours across the different limits and proposed guidelines for the design of low-Mach schemes.
However, these studies have primarily focused on specific discretisations and/or only the convective limit.

In this paper, we review the low-Mach behaviour using the modified equations - the continuous Euler equations augmented with artificial diffusion terms - which are representative of a wide range of schemes in this class.
By considering both convective and acoustic effects, we show that three diffusion scalings naturally arise.
Single- and multiple-scale asymptotic analysis of these scalings shows that many of the important low-Mach features of this class of schemes can be reproduced in a straightforward manner in the continuous setting.

As an example, we show that many existing low-Mach Roe-type finite-volume schemes match one of these three scalings.
Our analysis corroborates previous analysis of these schemes, and we are able to refine previous guidelines on the design of low-Mach schemes by including both convective and acoustic effects.
Discrete analysis and numerical examples demonstrate the behaviour of minimal Roe-type schemes with each of the three scalings for convective, acoustic, and mixed flows.

==> appendices/ausm2fds_proof.tex <==
General form of AUSM scheme
\begin{equation}
\hat{f}=\left\{ f\right\}- \dot{c}/2 \llbracket \varphi \rrbracket - c_d \llbracket -p_d n
\end{equation}
\begin{equation}
\dot{c}=\dot{u}
\end{equation}
\begin{equation}
    \hat{f}=\left\{ f\right\}- \left|A\right|\llbracket q\rrbracket=
    \dot{u}I\llbracket \varphi\rrbracket
    +\varphi 
    \left( \begin{matrix} \nu _p^u & \nu_u^u \end{matrix}\right)\left(
   \llbracket p\rrbracket \\
   \llbracket u \rrbracket 
    \right)
    +\left( \begin{matrix} 0\\1\\0\\0\end{matrix}\right)
    \left( \begin{matrix} \nu _p^p& \nu_u^p \end{matrix}\right)\left(
   \llbracket p\rrbracket \\
   \llbracket u \rrbracket 
    \right)
\end{equation}
where
\begin{equation}
    \varphi =\rho \left(\begin{matrix}
    1 \\ u \\ v \\ h
    \end{matrix}
    \right)
\end{equation}
Define
\begin{equation}
    \llbracket p\rrbracket= \rho a \llbracket \phi \rrbracket
\end{equation}
\begin{equation}
    \hat{f}=\left\{f\right\}-
    \left(
   \begin{matrix} 
   \dfrac{u}{2} \llbracket \rho \rrbracket+
   \nu_u^u\rho \llbracket u \rrbracket+
   \nu_p^u\rho \llbracket p \rrbracket \\
   \dfrac{u}{2} \llbracket \rho u \rrbracket+
   \nu_u^u\rho u \llbracket u \rrbracket+
   \nu_p^u\rho u \llbracket p \rrbracket +
   \nu_p^p\llbracket p\rrbracket+
   \nu_u^p\llbracket u\rrbracket \\
   \dfrac{u}{2} \llbracket \rho v\rrbracket+
   \nu_u^u\rho v \llbracket u \rrbracket+
   \nu_p^u\rho v \llbracket p \rrbracket \\
   \dfrac{u}{2} \llbracket \rho h\rrbracket+
   \nu_u^u\rho h \llbracket u \rrbracket+
   \nu_p^u\rho h \llbracket p \rrbracket
   \end{matrix} 
    \right)
\end{equation}

\begin{equation}
    \hat{f}=\left\{f\right\}-
    \left(
    \begin{matrix}
    \dfrac{u}{2} & 0 & 0 & 0 \\
    0 & \dfrac{u}{2} & 0 & 0 \\
    0 & 0 & \dfrac{u}{2} & 0 \\
    0 & 0 & 0 & \dfrac{u}{2} \\
    \end{matrix}
    \right)
    \left(
   \begin{matrix}
   \llbracket \rho \rrbracket \\
   \llbracket \rho u \rrbracket \\
   \llbracket \rho v \rrbracket \\
   \llbracket \rho h\rrbracket \\
   \end{matrix} 
    \right)
-
    \left(\begin{matrix}
     \nu_p^u \rho & \nu_u^u \rho \\
     \nu_p^u \rho u &\nu_p^p & \nu_u^u \rho u +\nu_u^p \\
     \nu_p^u \rho v & \nu_u^u \rho v  \\
     \nu_p^u \rho h & \nu_u^u \rho h \\
    \end{matrix}\right)
   \begin{matrix}
   \llbracket p \rrbracket
   \llbracket u \rrbracket
   \end{matrix} 
\end{equation}
Transformation jacobians
\begin{equation}
\dfrac{\partial q^s}{\partial q^c}=
\dfrac{1}{\rho a}\left( \begin{matrix}
\Gamma k & -\Gamma u & -\Gamma v & \Gamma \\
-u a &  a & 0 & 0 \\
-v a &  0 & a & 0 \\
\Gamma k -a^2 & -\Gamma u & -\Gamma v & \Gamma
\end{matrix}\right)
\end{equation}
\begin{equation}
\dfrac{\partial \varphi}{\partial q^s}=
\dfrac{\rho}{a}\left( \begin{matrix}
1 &  0 & 0 & -1 \\
 u &  a & 0 & -u \\
v  &  0 & a & -v \\
\dfrac{\gamma a^2}{\Gamma}+k & u a & v a& -k
\end{matrix}
\right)
\end{equation}
Note
\begin{equation}
\dfrac{\partial q^s}{\partial q^c}
\dfrac{\partial \varphi}{\partial q^s}=
\left(
\begin{matrix}
\gamma & 0 & 0 & 0 \\
     0 & 1 & 0 & 0 \\
     0 & 0 & 1 & 0 \\
     \gamma-1 & 0 & 1 & 0
\end{matrix}
\right)
\end{equation}
\begin{equation}
   A\llbracket q\rrbracket  \left[
   \dot{u} 
   \left(
   \begin{matrix}
    \gamma & 0 & 0 & 1\\
    0 & 1 & 0 & 0 \\
    0 & 0 & 1 & 0 \\
    \gamma-1 &  0 & 0 & 1
    \end{matrix}
    \right)
    +
    \left(
   \begin{matrix}
    \rho a^2 \nu_p^u & a \nu_u^u & 0 & 0\\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0
    \end{matrix}
    \right)
    +
    \left(
   \begin{matrix}
    -\Gamma \frac{u}{a}\\
    1 \\
    0 \\
    -\Gamma \dfrac{u}{a}
    \end{matrix}
    \right)\left(\begin{matrix} 0 & a \nu_p^p & \dfrac{\nu_u^p}{\rho} & 0\end{matrix}\right)
    \right]
    \left(
    \begin{matrix}
    \llbracket \phi \rrbracket \\
    \llbracket u \rrbracket \\
    \llbracket v \rrbracket \\
    \llbracket \zeta \rrbracket \\
    \end{matrix} 
    \right)
\end{equation}
\subsection{$\phi$ equation}
\begin{equation}
\left(\dot{u}\gamma\left(1-\nu_p^p\right)+ \rho a^2 \nu_p^u \right)\llbracket \phi \rrbracket
+\left( a\nu_u^u -\Gamma \nu_u^p \dfrac{u}{a}\right)\llbracket u\rrbracket
\end{equation}
\subsection{$u$ equation}
\begin{equation}
\left(a \nu_p^p\right)\llbracket \phi \rrbracket
+\left( \dot{u} + \dfrac{\nu_u^p}{\rho}\right)\llbracket u\rrbracket
\end{equation}
\subsection{$v$ equation}
\begin{equation}
\dot{u}\llbracket v\rrbracket
\end{equation}
\subsection{$\zeta$ equation}
\begin{equation}
\left(\dot{u}\left(\gamma-1\right)- \Gamma u \nu_p^p \right)\llbracket \phi \rrbracket 
- \dfrac{\gamma u \nu _u^p}{\rho a}\llbracket u \rrbracket + u\llbracket \zeta \rrbracket
\end{equation}
\begin{equation}
\dot{u}\left(\gamma-1\right)\left(1- \nu_p^p \right)\llbracket \phi \rrbracket 
- \dfrac{\gamma u \nu _u^p}{\rho a}\llbracket u \rrbracket + u\llbracket \zeta \rrbracket
\end{equation}


\subsection{Introduce symmetrising variables}
Proceed column by column
\begin{equation}
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \varphi \left(\begin{matrix}\nu_p^u && \nu_u^u \end{matrix}\right)\left(\begin{matrix}
   \llbracket p\rrbracket \\
   \llbracket u \rrbracket \end{matrix}\right)=
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \varphi \left(\begin{matrix}\rho a \nu_p^u && \nu_u^u \end{matrix}\right)\left(\begin{matrix}
   \llbracket \phi \rrbracket \\
   \llbracket u \rrbracket \end{matrix}\right)
\end{equation}
\begin{equation}
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \varphi =
   \dfrac{\rho}{\rho a}\left( 
  \begin{matrix}
  \Gamma k & -\Gamma u & -\Gamma v & \Gamma \\
  -u a & a & 0 & 0\\
  -v a & 0 & a & 0 \\
  \Gamma h -k & -\Gamma a & -\Gamma v & \Gamma
  \end{matrix} 
   \right)
   \left(
   \begin{matrix}
   1 \\ u \\ v \\ h
   \end{matrix}
   \right)=
   \dfrac{\Gamma}{a}\left( \begin{matrix}
   h-k \\ 0 \\ 0 \\ h-k-\dfrac{a^2}{\Gamma} 
   \end{matrix}\right)
\end{equation}
Note
\begin{equation}
    h-k= \dfrac{a^2}{\Gamma}
\end{equation}
hence
\begin{equation}
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \varphi =
   \left( \begin{matrix}
   a \\ 0 \\ 0 \\ 0
   \end{matrix}\right)
\end{equation}
\begin{equation}
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \varphi \left(\begin{matrix}\nu_p^u && \nu_u^u \end{matrix}\right)\left(\begin{matrix}
   \llbracket p\rrbracket \\
   \llbracket u \rrbracket \end{matrix}\right)=
   \left( \begin{matrix}
   1 \\ 0 \\ 0 \\ 0
   \end{matrix}\right)
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \varphi \left(\begin{matrix}\rho a \rho a^2 \nu_p^u && a \nu_u^u \end{matrix}\right)\left(\begin{matrix}
   \llbracket \phi \rrbracket \\
   \llbracket u \rrbracket \end{matrix}\right)
\end{equation}


\begin{equation}
   \left( \dfrac{\partial q^s}{\partial q^c}\right) 
  \left(\begin{matrix}0\\1\\0\\0\end{matrix}\right) 
   \left(\begin{matrix}\nu_p^u && \nu_u^u \end{matrix}\right)\left(\begin{matrix}
   \llbracket p\rrbracket \\
   \llbracket u \rrbracket \end{matrix}\right)=
   \left( \dfrac{\partial q^s}{\partial q^c}\right) 
  \left(\begin{matrix}0\\1\\0\\0\end{matrix}\right) 
   \left(\begin{matrix}\rho a \nu_p^u && \nu_u^u \end{matrix}\right)\left(\begin{matrix}
   \llbracket \phi \rrbracket \\
   \llbracket u \rrbracket \end{matrix}\right)
\end{equation}
\begin{equation}
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \left(\begin{matrix}
   0 \\ 1 \\ 0 \\ 0 \end{matrix}\right) =
   \dfrac{\rho}{\rho a}\left( 
  \begin{matrix}
  \Gamma k & -\Gamma u & -\Gamma v & \Gamma \\
  -u a & a & 0 & 0\\
  -v a & 0 & a & 0 \\
  \Gamma h -k & -\Gamma a & -\Gamma v & \Gamma
  \end{matrix} 
   \right)
   \left(
   \begin{matrix}
   0 \\ 1 \\ 0 \\ 0
   \end{matrix}
   \right)=
   \dfrac{1}{\rho a}\left( \begin{matrix}
   -\Gamma u \\ a \\ 0 \\ -\Gamma u 
   \end{matrix}\right)
\end{equation}
\begin{equation}
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \left(\begin{matrix}
  0 \\ 1 \\ 0 \\ 0  \end{matrix}\right)\left(\begin{matrix}
   \llbracket p\rrbracket \\
   \llbracket u \rrbracket \end{matrix}\right)=
   \dfrac{1}{\rho a}\left( \begin{matrix}
   -\Gamma u \\ a \\ 0 \\ -\Gamma u
   \end{matrix}\right)
   \left( \dfrac{\partial q^s}{\partial q^c}\right) \varphi \left(\begin{matrix}\rho a^2 \nu_p^u && a \nu_u^u \end{matrix}\right)\left(\begin{matrix}
   \llbracket \phi \rrbracket \\
   \llbracket u \rrbracket \end{matrix}\right)
\end{equation}

==> appendices/ausm_eigenvalues.tex <==

Spectral radius of upwind term:
\begin{equation}
    u : 3,
    \quad
    \gamma u : 1
\end{equation}
Spectral radius of interface velocity diffusion term:
\begin{equation}
    0 : 3,
    \quad
    \rho a^2 \nu_p : 1
\end{equation}
Spectral radius of interface pressure diffusion term:
\begin{equation}
    0 : 3,
    \quad
    \frac{\mu_u - \rho u \mu_p (\gamma-1)}{\rho} : 1
\end{equation}
Spectral radius of the combined upwinding and interface velocity diffusion:
\begin{equation}
    u : 3,
    \quad
    \gamma u + \rho a^2 \nu_p : 1
\end{equation}
Spectral radius of the combined interface velocity and pressure diffusion:
\begin{equation}
\begin{split}
    0 : 2 \\
    \frac{\mu_u - \rho u \mu_p (\gamma-1) + \rho^2 a^2 \nu_p}{2\rho} \\
    \pm \frac{\sqrt{
    \rho^4 a^4 \nu_p^2
    -2 \rho^3 a^2 u \nu_p ( \gamma - 1) \mu_p
    +2 \rho^2 a^2 ( 2 \nu_u \mu_p - \nu_p \mu_u )
    + ( \rho u \mu_p ( \gamma - 1 ) - \mu_u )^2
    }}{2\rho}
\end{split}
\end{equation}
Spectral radius of the full diffusive flux jacobian:
\begin{equation}
\begin{split}
    u : 2 \\
    \frac{\mu_u - \rho u \mu_p (\gamma-1) + \rho^2 a^2 \nu_p + \rho u (\gamma+1)}{2\rho} \\
    \pm \frac{\sqrt{
    \rho^4 a^4 \nu_p^2
    -2\rho^3 a^2 u \nu_p ( \gamma - 1 )( \mu_p - 1 )
    + 2\rho^2 a^2 ( 2 \nu_u \mu_p - \nu_p \mu_u )
    + ( \rho u \mu_p ( \gamma - 1 ) - \mu_u )^2
    + 4 \rho u \mu_u ( \gamma - 1 )
%   + \rho^2 u^2 ( \gamma - 1 )^2 ( \mu_p - 1 )^2
%   - 2\rho u \mu_u ( \gamma - 1 )( \mu_p + 1 )
%   + \mu_u^2
    }}{2\rho}
\end{split}
\end{equation}

==> appendices/ausm_scheme_comparison.tex <==
\subsection{AUSM$^+$-up}
The interface velocity in AUSM+up is:
\begin{equation}
    u_{1/2} =  a\mathcal{M}^{+}_{(4)}(M_L)
             + a\mathcal{M}^{-}_{(4)}(M_R)
             - \frac{1-M^2}{4 f_a} \frac{\llbracket p \rrbracket}{\rho a}
\end{equation}
Where $f_a=M_0(2-M_0)$, and $M_0$ is the local Mach number clamped between $1$ and a cut-off value $M_{co}$.
Any arithmetic coefficients have been taken as the values given in the original paper.
The fourth order Mach splittings $\mathcal{M}^{\pm}_{(4)}$ are given, for subsonic flow, by:
\begin{equation}
    \mathcal{M}^{\pm}_{(4)}(M) = \pm \frac{1}{8}(3 \pm 4M + M^4)
\end{equation}
Substituting (\ref{eq:mach_splitting_4th}) into (\ref{eq:ausmpup:interface_velocity}) and discarding higher order terms in $M$, the low Mach number approximation to the interface velocity is:
\begin{equation}
    u_{1/2} = \{u\} - \frac{\llbracket p \rrbracket}{8\rho a M} + \mathcal{O}(M^3)
\end{equation}
From which it can be see that:
\begin{equation}
    \nu_u \approx 0,
    \quad
    \nu_p = \frac{1}{4\rho a M} \sim \mathcal{O}(M^0)
\end{equation}
The interface pressure is given by:
\begin{equation}
    p_{1/2} =  \mathcal{P}^{+}_{(5)}(M_L)p_L
             + \mathcal{P}^{-}_{(5)}(M_R)p_R
             - \frac{3}{4}\mathcal{P}^{+}_{(5)}(M_L)\mathcal{P}^{-}_{(5)}(M_R)\rho f_a a \llbracket u \rrbracket
\end{equation}
The calculation of the fifth order pressure splittings $\mathcal{P}^{\pm}_{(5)}$ relies on a parameter $\alpha$ which, at low Mach number is approximately $-\frac{3}{4}$.
Using this approximation, the pressure splittings are:
\begin{equation}
    \mathcal{P}^{\pm}_{(5)}(M) = \frac{1}{4} ( 2 \pm 5M^3 \mp 3M^5 )
\end{equation}
Substituting (\ref{eq:pressure_splitting_5th_convective}) into (\ref{eq:ausmpup:interface_pressure}) and discarding higher order terms in $M$, the low Mach number approximation to the interface pressure is:
\begin{equation}
    p_{1/2} \approx \{p\} - \bigg( \frac{3\rho a M}{8} + \frac{15\rho a M^2}{4} \bigg)\llbracket u \rrbracket + \mathcal{O}(M^4)
\end{equation}
The second term in the brackets is an order of $M$ smaller than the first, so we neglect it in the limit to find:
\begin{equation}
    \mu_p \approx 0,
    \quad
    \mu_p \approx -\frac{3\rho a M}{8} \sim \mathcal{O}(M^0)
\end{equation}
Collecting (\ref{eq:ausmpup_nu_convective}) and (\ref{eq:ausmpup_mu_convective}) together, the diffusion matrix of AUSM$^+$-up scales as:
\begin{equation}
    \underline{\underline{A}} \sim \mathcal{O}
    \begin{matrix}
    \begin{pmatrix}
        M^{-2} & 0     \\
        0      & M^{0} \\
    \end{pmatrix}
    \end{matrix}
\end{equation}
This is a diagonal approximation to the convective limit diffusion matrix (\ref{eq:convective_diffusion_scaling}).
This result is unsurprising given the use of a discrete asymptotic analysis in the derivation of AUSM$^+$-up, and almost 15 years of evidence of AUSM$^+$-up producing satisfactory results for convective low Mach number problems.
In the original paper, Liou recognised that the asymptotic analysis relies on the assumption of a uniform background pressure, and recommended that for situations where this assumption does not hold - for example shock tube problems - the low Mach number scaling factor $f_a$ should be fixed equal to one.
In this case, the diagonal coefficients $\nu_p$ and $\mu_u$ decrease and increase by an order of $M$ respectively, and the approximation $\alpha\approx-\frac{3}{4}$ is no longer valid.
The pressure splittings are now:
\begin{equation}
    \mathcal{P}^{\pm}_{(5)}(M) = \frac{1}{16} ( 8 \pm 15M \mp 10M^3 \pm 3M^5 )
\end{equation}
The resulting diffusion coefficients are:
\begin{equation}
    \nu_u \approx 0,
    \quad
    \nu_p = \frac{1}{4\rho a} \sim \mathcal{O}(M^1)
\end{equation}
\begin{equation}
    \mu_p \approx 0,
    \quad
    \mu_p \approx -\frac{21\rho a}{16} \sim \mathcal{O}(M^{-1})
\end{equation}
and the diffusion matrix scales now as:
\begin{equation}
    \underline{\underline{A}} \sim \mathcal{O}
    \begin{matrix}
    \begin{pmatrix}
        M^{-1} & 0      \\
        0      & M^{-1} \\
    \end{pmatrix}
    \end{matrix}
\end{equation}
Which is a diagonal approximation of the acoustic limit diffusion matrix (\ref{eq:acoustic_diffusion_scaling}), showing that with $f_a=1$, AUSM$^+-up$ is not only suitable for low Mach number shock tube problems, but also acoustic problems where the background pressure is constant.


==> appendices/interface_massflux.tex <==

We consider AUSM fluxes which use an interface mass flow which cannot be defined as in equation (\ref{eq:interface_mass_flow}).
Equations (\ref{eq:ausm_form2}), (\ref{eq:interface_up}) and (\ref{eq:ausm_form3}) remain the same, except for $u_{1/2}$ being replaced with $\dot{m}_{1/2}$ and $\varphi=(1, u, v, h)$.
The diffusion on the interface pressure remains unchanged from equation (\ref{eq:interface_up_diffusion}), however we add a density diffusion term to the definition of the interface mass flow, in addition to the velocity and pressure diffusion terms:
\begin{equation}
    \dot{m}_d = \varrho_p \llbracket p \rrbracket + \varrho_u \llbracket u \rrbracket + \varrho_{\rho} \llbracket \rho \rrbracket
\end{equation}
The diffusive flux Jacobian in entropy variables, equivalent to equation (\ref{eq:ausm_diffusion_symmetric}) is:
\begin{equation} \label{eq:slau_jacobian}
    \Bigg[
    \frac{\dot{m}}{\rho}
    \begin{matrix}
        \begin{pmatrix}
            \Gamma & 0 & 0 & 1 \\
            0        & 1 & 0 & 0 \\
            0        & 0 & 1 & 0 \\
            \Gamma & 0 & 0 & 1
        \end{pmatrix}
    \end{matrix}
    +
    \begin{matrix}
        \begin{pmatrix}
            a^2\varrho_p + \varrho_{\rho} & a^2\varrho_u & 0 & -\varrho_{\rho} \\
            0                             & 0            & 0 & 0 \\
            0                             & 0            & 0 & 0 \\
            0                             & 0            & 0 & 0
        \end{pmatrix}
    \end{matrix}
    +
    \begin{matrix}
        \begin{pmatrix}
            -\Gamma u \\
            1/\rho \\
            0 \\
            -\Gamma u \\
        \end{pmatrix}
    \end{matrix}
    \begin{matrix}
        \begin{pmatrix}
            \mu_p & \mu_u & 0 & 0
        \end{pmatrix} \\
        \mbox{} \\
        \mbox{} \\
        \mbox{}
    \end{matrix}
    \Bigg]
    \begin{matrix}
        \begin{pmatrix}
            \llbracket p \rrbracket \\
            \llbracket u \rrbracket \\
            \llbracket v \rrbracket \\
            \llbracket s \rrbracket
        \end{pmatrix}
    \end{matrix}
\end{equation}
The equations for $u$, $v$ and $s$ remain unchanged compared to equation (\ref{eq:ausm_diffusion_symmetric}), as does the contribution of the interface pressure diffusion to the $p$ equation.
The (1,1) and (1,4) elements of the first two matrix terms are modified compared to equation (\ref{eq:ausm_diffusion_symmetric}).
These additional terms amount to:
\begin{equation} \label{eq:massflow_extra_term}
    \frac{\dot{m}}{\rho} - \varrho_{\rho}
\end{equation}
being subtracted from the (1,1) element, and added to the (1,4) element of the complete Jacobian.
If the two terms in equation (\ref{eq:massflow_extra_term}) are approximately equal at low Mach number, then the additional terms cancel, and the interface mass flow form is equivalent to the interface velocity form.
In the SLAU flux:
\begin{equation} \label{eq:slau_density_diffusion}
    \varrho_{\rho} \approx \frac{\{\dot{m}\}}{\{\rho\}}
\end{equation}
so the additional terms (\ref{eq:massflow_extra_term}) are approximately equal, and the Jacobian (\ref{eq:slau_jacobian}) can be considered equivalent to the interface velocity form (\ref{eq:ausm_diffusion_symmetric}).



==> appendices/non-diagonal_limit_equations.tex <==

\subsection{Roe scheme}

Limit equations at convective limit with convective diffusion for Roe.
\begin{subequations}
    \begin{align}
        \partial_t\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = \gamma\ord{p}{0}\Big( \frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{2} + \mu_{12}\partial_{xx}\ord{u}{0} \Big) \\
        \ord{\rho}{0}\partial_t\ord{u}{0} + \partial_x\ord{p}{2} + \ord{\rho u}{0}\partial_x\ord{u}{0} & = \ord{\rho}{0}\mu_u|u|\partial_{xx}\ord{u}{0} + \mu_{21}\partial_{xx}\ord{p}{2} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_t\ord{v}{0}                           +      \ord{u}{0}\partial_x\ord{v}{0} & = \mu_u|u|\partial_{xx}\ord{v}{0} \\
        \partial_t\ord{s}{0}                           +      \ord{u}{0}\partial_x\ord{s}{0} & = \mu_u|u|\partial_{xx}\ord{s}{0}
    \end{align}
\end{subequations}

Limit equations at acoustic limit with convective diffusion for Roe.
\begin{subequations}
    \begin{align}
        0 & = \gamma\ord{p}{0}\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{1} \\
        \ord{\rho}{0}\partial_{\tau}\ord{u}{0} + \partial_x\ord{p}{1} & = \mu_{21}\partial_{xx}\ord{p}{1} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_{\tau}\ord{v}{0} & = 0 \\
        \partial_{\tau}\ord{s}{0} & = 0
    \end{align}
\end{subequations}

Limit equations at convective limit with mixed diffusion for Roe.
\begin{subequations}
    \begin{align}
        \partial_t\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & =  \gamma\ord{p}{0}\mu_{12}\partial_{xx}\ord{u}{0} \\
        \ord{\rho}{0}\partial_t\ord{u}{0} + \partial_x\ord{p}{2} + \ord{\rho u}{0}\partial_x\ord{u}{0} & = \ord{\rho}{0}\mu_u|u|\partial_{xx}\ord{u}{0} + \mu_{21}\partial_{xx}\ord{p}{2} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_t\ord{v}{0}                           +      \ord{u}{0}\partial_x\ord{v}{0} & = \mu_u|u|\partial_{xx}\ord{v}{0} \\
        \partial_t\ord{s}{0}                           +      \ord{u}{0}\partial_x\ord{s}{0} & = \mu_u|u|\partial_{xx}\ord{s}{0}
    \end{align}
\end{subequations}

Limit equations at acoustic limit with mixed diffusion for Roe.
\begin{subequations}
    \begin{align}
        \partial_{\tau}\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = \gamma\ord{p}{0}\Big(\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{1} + \mu_{12}\partial_{xx}\ord{u}{0}\Big) \\
        \ord{\rho}{0}\partial_{\tau}\ord{u}{0} + \partial_x\ord{p}{1} & = \mu_{21}\partial_{xx}\ord{p}{1} \\
        \partial_{\tau}\ord{v}{0} & = 0 \\
        \partial_{\tau}\ord{s}{0} & = 0
    \end{align}
\end{subequations}

\subsection{Liou-Steffen splitting}

Limit equations at convective limit with convective diffusion for Liou-Steffen.
\begin{subequations}
    \begin{align}
        \partial_t\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = \gamma\ord{p}{0}\Big( \frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{2} + \mu_{12}\partial_{xx}\ord{u}{0} \Big) \\
        \ord{\rho}{0}\partial_t\ord{u}{0} + \partial_x\ord{p}{2} + \ord{\rho u}{0}\partial_x\ord{u}{0} & = \ord{\rho}{0}\mu_u|u|\partial_{xx}\ord{u}{0} + \mu_{21}\partial_{xx}\ord{p}{2} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_t\ord{v}{0}                           +      \ord{u}{0}\partial_x\ord{v}{0} & = \mu_u|u|\partial_{xx}\ord{v}{0} \\
        \partial_t\ord{s}{0}                           +      \ord{u}{0}\partial_x\ord{s}{0} & = \ord{\rho}{0}\gamma R\mu_u|u|\partial_{xx}\ord{T}{0}
    \end{align}
\end{subequations}

Limit equations at acoustic limit with convective diffusion for Liou-Steffen.
\begin{subequations}
    \begin{align}
        0 & = \gamma\ord{p}{0}\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{1} \\
        \ord{\rho}{0}\partial_{\tau}\ord{u}{0} + \partial_x\ord{p}{1} & = \mu_{21}\partial_{xx}\ord{p}{1} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_{\tau}\ord{v}{0} & = 0 \\
        \partial_{\tau}\ord{s}{0} & = 0
    \end{align}
\end{subequations}

Limit equations at convective limit with mixed diffusion for Liou-Steffen.
\begin{subequations}
    \begin{align}
        \partial_t\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & =  \gamma\ord{p}{0}\mu_{12}\partial_{xx}\ord{u}{0} \\
        \ord{\rho}{0}\partial_t\ord{u}{0} + \partial_x\ord{p}{2} + \ord{\rho u}{0}\partial_x\ord{u}{0} & = \ord{\rho}{0}\mu_u|u|\partial_{xx}\ord{u}{0} + \mu_{21}\partial_{xx}\ord{p}{2} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_t\ord{v}{0}                           +      \ord{u}{0}\partial_x\ord{v}{0} & = \mu_u|u|\partial_{xx}\ord{v}{0} \\
        \partial_t\ord{s}{0}                           +      \ord{u}{0}\partial_x\ord{s}{0} & = \ord{\rho}{0}\gamma R\mu_u|u|\partial_{xx}\ord{T}{0}
    \end{align}
\end{subequations}

Limit equations at acoustic limit with mixed diffusion for Liou-Steffen.
\begin{subequations}
    \begin{align}
        \partial_{\tau}\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = \gamma\ord{p}{0}\Big(\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{1} + \mu_{12}\partial_{xx}\ord{u}{0}\Big) \\
        \ord{\rho}{0}\partial_{\tau}\ord{u}{0} + \partial_x\ord{p}{1} & = \mu_{21}\partial_{xx}\ord{p}{1} \\
        \partial_{\tau}\ord{v}{0} & = 0 \\
        \partial_{\tau}\ord{s}{0} & = 0
    \end{align}
\end{subequations}

\subsection{Zha-Bilgen splitting}

Limit equations at convective limit with convective diffusion for Zha-Bilgen.
\begin{subequations}
    \begin{align}
        \partial_t\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = \ord{p}{0}\Big( \frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{2} + \mu_{12}\partial_{xx}\ord{u}{0} \Big) \\
        \ord{\rho}{0}\partial_t\ord{u}{0} + \partial_x\ord{p}{2} + \ord{\rho u}{0}\partial_x\ord{u}{0} & = \ord{\rho}{0}\mu_u|u|\partial_{xx}\ord{u}{0} + \mu_{21}\partial_{xx}\ord{p}{2} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_t\ord{v}{0}                           +      \ord{u}{0}\partial_x\ord{v}{0} & = \mu_u|u|\partial_{xx}\ord{v}{0} \\
        \partial_t\ord{s}{0}                           +      \ord{u}{0}\partial_x\ord{s}{0} & = \mu_u|u|\partial_{xx}\ord{s}{0} - \ord{p}{0}(\gamma-1)\Big(\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{2} + \mu_{12}\partial_{xx}\ord{u}{0}\Big) \\
    \end{align}
\end{subequations}

Limit equations at acoustic limit with convective diffusion for Zha-Bilgen.
\begin{subequations}
    \begin{align}
        0 & = \ord{p}{0}\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{1} \\
        \ord{\rho}{0}\partial_{\tau}\ord{u}{0} + \partial_x\ord{p}{1} & = \mu_{21}\partial_{xx}\ord{p}{1} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_{\tau}\ord{v}{0} & = 0 \\
        \partial_{\tau}\ord{s}{0} & = -\ord{p}{0}(\gamma-1)\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{1}
    \end{align}
\end{subequations}

Limit equations at convective limit with mixed diffusion for Zha-Bilgen.
\begin{subequations}
    \begin{align}
        \partial_t\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & =  \ord{p}{0}\mu_{12}\partial_{xx}\ord{u}{0} \\
        \ord{\rho}{0}\partial_t\ord{u}{0} + \partial_x\ord{p}{2} + \ord{\rho u}{0}\partial_x\ord{u}{0} & = \ord{\rho}{0}\mu_u|u|\partial_{xx}\ord{u}{0} + \mu_{21}\partial_{xx}\ord{p}{2} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_t\ord{v}{0}                           +      \ord{u}{0}\partial_x\ord{v}{0} & = \mu_u|u|\partial_{xx}\ord{v}{0} \\
        \partial_t\ord{s}{0}                           +      \ord{u}{0}\partial_x\ord{s}{0} & = \mu_u|u|\partial_{xx}\ord{s}{0} - \ord{p}{0}(\gamma-1)\mu_{12}\partial_{xx}\ord{u}{0} \\
    \end{align}
\end{subequations}

Limit equations at acoustic limit with mixed diffusion for Zha-Bilgen.
\begin{subequations}
    \begin{align}
        \partial_{\tau}\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = \ord{p}{0}\Big(\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{1} + \mu_{12}\partial_{xx}\ord{u}{0}\Big) \\
        \ord{\rho}{0}\partial_{\tau}\ord{u}{0} + \partial_x\ord{p}{1} & = \mu_{21}\partial_{xx}\ord{p}{1} \\
        \partial_{\tau}\ord{v}{0} & = 0 \\
        \partial_{\tau}\ord{s}{0} & = 0
    \end{align}
\end{subequations}

\subsection{Toro-Vasquez splitting}

Limit equations at convective limit with convective diffusion for Toro-Vasquez.
\begin{subequations}
    \begin{align}
        \partial_t\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = 0 \\
        \ord{\rho}{0}\partial_t\ord{u}{0} + \partial_x\ord{p}{2} + \ord{\rho u}{0}\partial_x\ord{u}{0} & = \ord{\rho}{0}\mu_u|u|\partial_{xx}\ord{u}{0} + \mu_{21}\partial_{xx}\ord{p}{2} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_t\ord{v}{0}                           +      \ord{u}{0}\partial_x\ord{v}{0} & = \mu_u|u|\partial_{xx}\ord{v}{0} \\
        \partial_t\ord{s}{0}                           +      \ord{u}{0}\partial_x\ord{s}{0} & = -a^2\mu_u|u|\partial_{xx}\ord{\rho}{0} - \gamma\ord{p}{0}\Big( \frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{2} + \mu_{12}\partial_{xx}\ord{u}{0} \Big)
    \end{align}
\end{subequations}

Limit equations at acoustic limit with convective diffusion for Toro-Vasquez.
\begin{subequations}
    \begin{align}
        \partial_{\tau}\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = 0 \\
        \ord{\rho}{0}\partial_{\tau}\ord{u}{0} + \partial_x\ord{p}{1} & = \mu_{21}\partial_{xx}\ord{p}{1} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_{\tau}\ord{v}{0} & = 0 \\
        \partial_{\tau}\ord{s}{0} & =  -\gamma\ord{p}{0}\frac{\mu_{11}}{\ord{\rho}{0}|v|}\partial_{xx}\ord{p}{1}
    \end{align}
\end{subequations}

Limit equations at convective limit with mixed diffusion for Toro-Vasquez.
\begin{subequations}
    \begin{align}
        \partial_t\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = 0 \\
        \ord{\rho}{0}\partial_t\ord{u}{0} + \partial_x\ord{p}{2} + \ord{\rho u}{0}\partial_x\ord{u}{0} & = \ord{\rho}{0}\mu_u|u|\partial_{xx}\ord{u}{0} + \mu_{21}\partial_{xx}\ord{p}{2} + \ord{\rho}{0}|v|\mu_{22}\partial_{xx}\ord{u}{0} \\
        \partial_t\ord{v}{0}                           +      \ord{u}{0}\partial_x\ord{v}{0} & = \mu_u|u|\partial_{xx}\ord{v}{0} \\
        \partial_t\ord{s}{0}                           +      \ord{u}{0}\partial_x\ord{s}{0} & = -a^2\mu_u|u|\partial_{xx}\ord{\rho}{0} - \gamma\ord{p}{0}\mu_{12}\partial_{xx}\ord{u}{0}
    \end{align}
\end{subequations}

Limit equations at acoustic limit with mixed diffusion for Toro-Vasquez.
\begin{subequations}
    \begin{align}
        \partial_{\tau}\ord{p}{0} + \gamma\ord{p}{0}\partial_x\ord{u}{0} & = 0 \\
        \ord{\rho}{0}\partial_{\tau}\ord{u}{0} + \partial_x\ord{p}{1} & = \mu_{21}\partial_{xx}\ord{p}{1} \\
        \partial_{\tau}\ord{v}{0} & = 0 \\
        \partial_{\tau}\ord{s}{0} & = 0
    \end{align}
\end{subequations}

==> appendices/non-dimensional_diffusion.tex <==
The full equations are:\\

Roe-type diffusion:
\begin{subequations}
    \begin{align}
        \mathcal{R}_p & =
            \phantom{\rho}\mu_u|u|\partial_{xx}p
                + \gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)
                \phantom{+\big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big)} \\
        \mathcal{R}_u & =
            \rho\mu_u|u|\partial_{xx}u
                \phantom{+ \gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)}
                +\big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big) \\
        \mathcal{R}_v & = \phantom{\rho}\mu_u|u|\partial_{xx}v \\
        \mathcal{R}_s & = \phantom{\rho}\mu_u|u|\partial_{xx}s
    \end{align}
\end{subequations}

Liou-Steffen diffusion:
\begin{subequations}
    \begin{align}
        \mathcal{R}_p & =
            \phantom{\rho}\mu_u|u|\partial_{xx}p
                + \gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)
                - M^2u(\gamma-1)\big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big) \\
        \mathcal{R}_u & =
            \rho\mu_u|u|\partial_{xx}u
                \phantom{+ \gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)}
                \phantom{M^2(\gamma-1)u}+ \big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big) \\
        \mathcal{R}_v & =
            \phantom{\rho}\mu_u|u|\partial_{xx}v \\
        \mathcal{R}_s & =
            \rho R\gamma\mu_u|u|\partial_{xx}T
                \phantom{\gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)}
                - M^2u(\gamma-1)\big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big) \\
    \end{align}
\end{subequations}

Zha-Bilgen diffusion:
\begin{subequations}
    \begin{align}
        \mathcal{R}_p & =
            \phantom{\rho}\mu_u|u|\partial_{xx}p
                \phantom{(-1)} + \gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)
                \phantom{+ \big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big)} \\
        \mathcal{R}_u & =
            \rho\mu_u|u|\partial_{xx}u
                \phantom{+ (\gamma-1)p\big(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\big)}
                + \big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big) \\
        \mathcal{R}_v & =
            \phantom{\rho}\mu_u|u|\partial_{xx}v \\
        \mathcal{R}_s & =
            \phantom{\rho}\mu_u|u|\partial_{xx}s
                - (\gamma-1)p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)
    \end{align}
\end{subequations}

Toro-Vasquez diffusion:
\begin{subequations}
    \begin{align}
        \mathcal{R}_p & =
            \phantom{-\rho}\mu_u|u|\partial_{xx}p
                \phantom{- \gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)}
                + M^2u(\gamma-1)\big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big) \\
        \mathcal{R}_u & =
            \phantom{-}\rho\mu_u|u|\partial_{xx}u
                \phantom{- \gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)}
                \phantom{M^2(\gamma-1)u}+ \big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big) \\
        \mathcal{R}_v & = \phantom{-\rho}\mu_u|u|\partial_{xx}v \\
        \mathcal{R}_s & = -a^2\mu_u|u|\partial_{xx}\rho
                - \gamma p\bigg(\frac{M^{\-2}}{\rho|v|}\mu_{11}\partial_{xx}p + \mu_{12}\partial_{xx}u\bigg)
                + M^2u(\gamma-1)\big(M^{\-2}\mu_{21}\partial_{xx}p + \rho|v|\mu_{22}\partial_{xx}u\big) \\
    \end{align}
\end{subequations}


==> backups/low_mach_asymptotes_conserved.tex <==

\textit{What is the point of this section? \\ To introduce the necessary theoretical background for the rest of the paper. The asymptotic solutions section is about the physical behaviour, the symmetrising variables section is on what this means for designing accurate numerical schemes. No original content except the stability estimates at the end.}

\subsection{Convective and acoustic asymptotic solutions}
We review the theoretical results for the asymptotic solutions for the Euler equations at low Mach number, as preparation for analysing numerical schemes in this regime later.
We follow closely the exposition of Muller99 **, highlighting the results most relevant to the current study. \\
First, all variables are non-dimensionalised using:
\begin{equation}
\begin{gathered}
    \tilde{\rho} = \frac{\rho}{\rho_{\infty}},
    \quad
    \tilde{\underline{u}} = \frac{\underline{u}}{u_{\infty}},
    \quad
    \tilde{\underline{x}} = \frac{\underline{x}}{L_{\infty}},
    \quad
    \tilde{e} = \frac{e}{a^2_{\infty}},
    \quad
    \tilde{h} = \frac{h}{a^2_{\infty}},
    \quad
    \tilde{p} = \frac{p}{\rho a^2_{\infty}},
    \quad
    \tilde{t} = \frac{t}{L_{\infty}/u_{\infty}}
\end{gathered}
\end{equation}
The Euler equations in conserved variables become:
\begin{subequations} \label{eq:euler}
\begin{align}
    \label{eq:euler_continuity}
    \partial_{\tilde{t}} \tilde{\rho} + \underline{\tilde{\nabla}}\cdot(\tilde{\rho} \underline{\tilde{u}}) = 0 \\
    \label{eq:euler_momentum}
    \partial_{\tilde{t}} (\tilde{\rho} \tilde{u}) + \underline{\tilde{\nabla}}\cdot(\tilde{\rho} \underline{\tilde{u}}\,\underline{\tilde{u}}) + \frac{1}{\tilde{M}^2}\underline{\tilde{\nabla}}\,\tilde{p} = 0 \\
    \label{eq:euler_energy}
    \partial_{\tilde{t}} \tilde{\rho} \tilde{e} + \underline{\tilde{\nabla}}\cdot(\tilde{\rho} \underline{\tilde{u}} \tilde{h}) = 0
\end{align}
\end{subequations}
Where $M=u_{\infty}/a_{\infty}$ is the reference Mach number.
Using $M$ as a small parameter, we treat system (\ref{eq:euler}) as a perturbation problem and expand all variables as power series of $M$:
\begin{equation} \label{eq:power_expansion}
    \psi(\underline{x},t,M) =     \psi_0 (\underline{x},t)
                             + M  \psi_1 (\underline{x},t)
                             + M^2\psi_2 (\underline{x},t)
                             + \mathcal{O}(M^3)
\end{equation}
The expansions (\ref{eq:power_expansion}) are inserted into the system (\ref{eq:euler}) and terms are grouped by powers of the parameter $M$.
First we examine the relations from the velocity equations \ref{eq:euler_velocity}, where the $1/M^2$ coefficient on the pressure gradient term means the lowest order terms are $M^{-2}$, $M^{-1}$ and $M^{0}$, leading to the following relations:
\begin{subequations} \label{eq:momentum_convective_timescale}
\begin{align}
    \label{eq:momentum_convective_0}
    \underline{\tilde{\nabla}}\,\tilde{p}_0 = 0 \\
    \label{eq:momentum_convective_1}
    \underline{\tilde{\nabla}}\,\tilde{p}_1 = 0 \\
    \label{eq:momentum_convective_2}
    \partial_{\tilde{t}} (\tilde{\rho} \tilde{u})_0 + \underline{\tilde{\nabla}}\cdot(\tilde{\rho} \underline{\tilde{u}}\,\underline{\tilde{u}})_0 + \underline{\tilde{\nabla}}\,\tilde{p}_2 = 0
\end{align}
\end{subequations}
Relations (\ref{eq:momentum_convective_0}) and (\ref{eq:momentum_convective_1}) imply that both the zeroth and first order terms for the pressure vary only in time, so for the pressure, the expansion (\ref{eq:power_expansion}) can be replaced with:
\begin{equation}
    \tilde{p}(\underline{\tilde{x}},\tilde{t},\tilde{M}) = \tilde{p}_0(\tilde{t}) + \tilde{M}^2\tilde{p}_2(\underline{\tilde{x}},\tilde{t}) + \mathcal{O}(\tilde{M}^3)
\end{equation}
with a spatially uniform background pressure, and spatial variations on the order of $\mathcal{O}(\tilde{M}^2)$, which essentially react only to the dynamic pressure of the leading order momentum in a Bernoulli type manner.
The divergence of the leading order velocity is constrained by:
\begin{equation} \label{eq:divergence_convective_timescale}
    \underline{\tilde{\nabla}}\cdot\underline{\tilde{u}}_0 = \frac{1}{\gamma \tilde{p}_0}d_{\tilde{t}}\tilde{p}_0
\end{equation}
meaning that the divergence is also spatially uniform and reacts everywhere instantaneously to temporal variations in the background pressure.
Acoustics are removed from the solution, leaving only convective effects.
Heuristically, this should not be surprising, given our choice of the convective timescale $L_{\infty}/u_{\infty}$ to non-dimensionalise the time derivatives in equation (\ref{eq:euler}).

Muller uses a two-timescale, one space scale asymptotic analysis to include acoustic effects, defining an additional non-dimensional time, $\tau$, scaled by the acoustic speed:
\begin{equation}
    \tau = \frac{t}{L_{\infty}/a_{\infty}} = \frac{\tilde{t}}{\tilde{M}}
\end{equation}
leading to the power series expansion:
\begin{equation} \label{eq:power_expansion_acoustic}
    \psi(\underline{\tilde{x}},\tilde{t},\tilde{M}) =             \psi_0 (\underline{\tilde{x}},\tilde{t},\tau)
                                                     + \tilde{M}  \psi_1 (\underline{\tilde{x}},\tilde{t},\tau)
                                                     + \tilde{M}^2\psi_2 (\underline{\tilde{x}},\tilde{t},\tau) + \mathcal{O}(\tilde{M}^3)
\end{equation}
The time derivatives at constant $\underline{\tilde{x}}$ and $\tilde{M}$ are now:
\begin{equation}
    \partial_{\tilde{t}} \psi\Big|_{\underline{\tilde{x}},\tilde{M}} = \big( \partial_{\tilde{t}} + \frac{1}{\tilde{M}}\partial_{\tau} \big) \psi
\end{equation}
Similiarly to the convective limit, the main results for the acoustic limit stem from the three lowest order relations from the momentum equation:
\begin{subequations} \label{eq:momentum_acoustic_timescale}
\begin{align}
    \label{eq:momentum_acoustic_0}
    \underline{\tilde{\nabla}}\,\tilde{p}_0 = 0 \\
    \label{eq:momentum_acoustic_1}
    \partial_{\tau}(\tilde{\rho}\tilde{u})_0 + \underline{\tilde{\nabla}}\,\tilde{p}_1 = 0 \\
    \label{eq:momentum_acoustic_2}
    \partial_{\tau}(\tilde{\rho}\tilde{u})_1 + \partial_{\tilde{t}} (\tilde{\rho} \tilde{u})_0 + \underline{\tilde{\nabla}}\cdot(\tilde{\rho} \underline{\tilde{u}}\,\underline{\tilde{u}})_0 + \underline{\tilde{\nabla}}\,\tilde{p}_2 = 0
\end{align}
\end{subequations}
The zeroth order pressure term is again constant in space, however the same is no longer true for the first order pressure term, which now varies with fluctuations on the acoustic timescale of the leading order momentum.
The second order pressure is still the relevant pressure for leading order momentum fluctuations on the convective time scale, but now is also related to the fluctuations of the first order momentum on the acoustic timescale.
With the two-timescale asymptotic expansion, the divergence of the leading order velocity is constrained by:
\begin{equation} \label{eq:divergence_acoustic_timescale}
    \underline{\tilde{\nabla}}\cdot\underline{\tilde{u}}_0 = \frac{1}{\gamma p_0}\big( d_{\tilde{t}}\tilde{p}_0 + \partial_{\tau}\tilde{p}_1 \big)
\end{equation}
and is now allowed to vary spatially through the acoustic-time derivative of the first order pressure. \\

To summarise the important points of this section, we have two asymptotic expansions of the inviscid Euler equations at low Mach number, one including acoustic effects, one not.
At the convective limit:
\begin{itemize}
    \item the non-dimensional pressure $\frac{p}{\rho_{\infty}a^2_{\infty}}$ has second order spatial variations with the dynamic pressure,
    \item the divergence of the leading order velocity is spatially uniform and reacts everywhere instantaneously to changes in the background pressure.
\end{itemize}
At the acoustic limit:
\begin{itemize}
    \item the non-dimensional pressure $\frac{p}{\rho_{\infty}a^2_{\infty}}$ has spatial variations due to the first order acoustic pressure and the second order dynamic pressure.
    \item the divergence of the leading order velocity varies in space with fluctuations on the acoustic timescale of the first order acoustic pressure.
\end{itemize}

Only the most relevant points of the asymptotics analysis have been presented here. For a more complete picture, see Muller99 ** and Muller (habilitation thesis), including the effects of diffusion, conduction and heat addition, and some implications for numerical schemes for these regimes.

\subsection{Asymptotic notation}
Before we continue, we clarify our use of asymptotic notation.
Up until now we have used the traditional definition of big-O ($\mathcal{O}$) as an upper bound, i.e.
\[f(M)\sim\mathcal{O}(M^n) \;\Rightarrow\; |f(M)|<c_f M^n \; \forall \; M<c_0\]
where $c_f$ and $c_0$ are constants that may depend on any flow condition or material property excluding the Mach number, although $c_0$ will usually be somewhere slightly smaller than 0.2, where compressibility effects become small.
For the rest of the paper we are concerned with finding (and designing) limit equations, where only the largest terms remain as $M\to0$, for which a bound is an insufficient metric.
For example, both terms in $f(M) = M^3 + M^2$ are $\mathcal{O}(M^2)$ as $M\to0$ under the definition above, however only $M^2$ remains in the limit equation.
Instead, we will use a stricter definition:
\begin{equation} \label{eq:asymptotic_order}
    f(M) \sim \mathcal{O}(M^n) \; \Rightarrow \; \exists \; c_f \in \mathbb{R}\; \textrm{s.t.}\; \forall \varepsilon>0 \;\exists\; \delta>0 \;\textrm{s.t.}\; | f(M) - c_f M^n |<\varepsilon \; \forall \: M<\delta
\end{equation}
We will also (mis)use the \textit{less-than-approximately} and \textit{greater-than-approximately} symbols to mean asymptotically smaller or larger than.
As we are concerned with the limit as $M\to0$, a higher order of M will be asymptotically smaller than a lower order of M, and vice-versa:
\begin{equation}
    \begin{split}
        g(M) \lesssim \mathcal{O}(M^n) \; & \Rightarrow \; g(M) \sim \mathcal{O}(M^m), \: m>n \\
        h(M) \gtrsim  \mathcal{O}(M^n) \; & \Rightarrow \; h(M) \sim \mathcal{O}(M^l), \: l<n
    \end{split}
\end{equation}
Lastly, where terms are independent of $M$ we use $\mathcal{O}(M^0)$ instead of $\mathcal{O}(1)$, to be clear we do not mean that the order of magnitude is necessarily on the order of unity.

\subsection{Symmetrising variables and artificial diffusion}
In this section we examine the implications of the above asymptotic analysis on the symmetrised Euler equations.
In particular, we are interested in the appropriate scaling of the artificial diffusion of a numerical scheme to achieve accurate solutions at the convective and acoustic limits.
The results for the single timescale convective limit are reproduced from Turkel's Annual Review article on low Mach number preconditioning **. We extend the analysis to the two timescale mixed convective/acoustic limit, as well as estimating the scaling of the spectral radius of the artificial diffusion at each limit. \\
The symmetrising variables are:
\begin{equation} \label{eq:symmetry_variables}
    d\underline{q}^s = ( d\phi, du, dv, d\zeta ),
    \quad
    d\phi = \frac{dp}{\rho a},
    \quad
    d\zeta = \frac{ads}{C_p} = \frac{dp - a^2d\rho}{\rho a}
\end{equation}
where $ds$ is the entropy variation.
The corresponding form of the $x$-split 2D Euler equations, with artificial diffusion matrix $A_{ij}$ is:
\begin{subequations} \label{eq:euler_symmetric}
    \begin{align}
        \label{eq:pressure_symmetric}
        \partial_t \phi + u\partial_x \phi + a\partial_x u & = A_{11}\partial_{xx}\phi + A_{12}\partial_{xx}u \\
        \label{eq:velocity_symmetric}
        \partial_t u    + a\partial_x \phi + u\partial_x u & = A_{21}\partial_{xx}\phi + A_{22}\partial_{xx}u \\
        \label{eq:vorticity_symmetric}
        \partial_t v                       + u\partial_x v & = A_{33}\partial_{xx}v \\
        \label{eq:entropy_symmetric}
        \partial_t s                       + u\partial_x s & = A_{44}\partial_{xx}s
    \end{align}
\end{subequations}
where the form of the artificial diffusion mirrors the form of the physical ($x$-split) flux Jacobian:
\begin{equation} \label{eq:symmetric_jacobian}
\frac{\partial \underline{f}^s}{\partial \underline{q}^s} =
\begin{matrix}
\begin{pmatrix}
u & a & 0 & 0 \\
a & u & 0 & 0 \\
0 & 0 & u & 0 \\
0 & 0 & 0 & u
\end{pmatrix}
\end{matrix}
\end{equation}
The flux Jacobian shows one of the main advantages of the symmetry variables, which is that they decouple the linearly degenerate vorticity and entropy fields from the pressure and normal velocity fields, which constitute the genuinely non-linear acoustic subsystem.
For the majority of this section we will only consider the acoustic subsystem, as this is the distinguishing feature between the low Mach number limits.
We call the normal velocity $du$ the velocity field, as it is the convecting velocity in the $x$-split fluxes, and we call the transverse velocity $dv$ the vorticity field, as it corresponds to the gradient $\frac{\partial v}{\partial x}$.

Turkel ** estimates the required scaling of the coefficients $A^c_{ij}$, $i,j=1,2$ in the convective limit by finding the order of the limit equations, given that the variables in equations (\ref{eq:pressure_symmetric}) and (\ref{eq:velocity_symmetric}) scale as:
\begin{equation} \label{eq:symmetric_convective_scaling}
    d\phi \sim \mathcal{O}(M),
    \quad
    du \sim \mathcal{O}(M^0),
    \quad
    a \sim \mathcal{O}(M^{-1})
\end{equation}
where the symmetric pressure $d\phi=\frac{dp}{\rho a}$ scales one order of $M$ lower than the non-dimensional pressure $\tilde{p}=\frac{p}{\rho a^2}$ used in the previous section.
To properly derive the continuous limit equations, we would also need to state whether we are using the convective ($dt\sim\mathcal{O}(M^0)$) or acoustic ($d\tau\sim\mathcal{O}(M^{1})$) timescale for the time derivative term.
However, as we are concerned with numerical schemes we consider this term a derived value which, for both unsteady and steady solvers, is calculated from the spatial residual and so is always included in the limit equations.
Using the above scaling (\ref{eq:symmetric_convective_scaling}), the largest terms on the left hand side of equations (\ref{eq:pressure_symmetric}) and (\ref{eq:velocity_symmetric}) in the convective limit are $\mathcal{O}(M^{-1})$ and $\mathcal{O}(M^0)$ respectively, so the coefficients $A^c_{11}$ and $A^c_{22}$ should be $\mathcal{O}(M^{-2})$ and $\mathcal{O}(M^0)$ respectively for the diagonal artificial diffusion terms to remain in the limit equations.
By the same argument, the off-diagonal coefficients should be $\mathcal{O}(M^{-1})$\footnote[2]{
    The off-diagonal coefficients can be asymptotically smaller, although in this case they will disappear from the limit equations as $M\to0$ and only the diagonal coefficients will remain.}.
The limit equations for the convective limit are then:
\begin{subequations} \label{eq:convective_limit_equations}
    \begin{align}
        \label{eq:convective_limit_pressure}
        \partial_t \phi                    + a\partial_x u & = A^c_{11}\partial_{xx}\phi + A^c_{12}\partial_{xx}u \\
        \label{eq:convective_limit_velocity}
        \partial_t u    + a\partial_x \phi + u\partial_x u & = A^c_{21}\partial_{xx}\phi + A^c_{22}\partial_{xx}u
    \end{align}
\end{subequations}
With diffusion matrix scaling as:
\begin{equation} \label{eq:convective_diffusion_scaling}
    \underline{\underline{A}}^c \sim \mathcal{O}
    \begin{matrix}
    \begin{pmatrix}
    M^{-2} & M^{-1} \\
    M^{-1} & M^0    \\
    \end{pmatrix}
    \end{matrix}
\end{equation}
The limit equations (\ref{eq:convective_limit_equations}) are almost identical to the governing equations of the Artificial Compressibility Method (**Chorin), which was the basis for much of the early work on low Mach number preconditioning **.
If converged to a steady state, the pressure equations (\ref{eq:convective_limit_pressure}) shows that the velocity divergence will be driven to zero (up to the value of the diffusion terms) as expected in the incompressible limit.

We now repeat to obtain the limit equations and correct scaling of the artificial diffusion in the two timescale limit.
At this limit, there are both convective and acoustic components, with different Mach number scalings.
The convective component scales identically to in the single timescale limit, so will require the artificial diffusion in (\ref{eq:convective_diffusion_scaling}) to be well balanced.
According to the analysis in section **, the scaling for the acoustic component of the two timescale limit is:
\begin{equation} \label{eq:symmetric_acoustic_scaling}
    d\phi \sim \mathcal{O}(M^0),
    \quad
    du \sim \mathcal{O}(M^0),
    \quad
    a \sim \mathcal{O}(M^{-1})
\end{equation}
Resulting in the limit equations:
\begin{subequations} \label{eq:acoustic_limit_equations}
    \begin{align}
        \label{eq:acoustic_limit_pressure}
        \partial_t \phi + a\partial_x u    & = A^a_{11}\partial_{xx}\phi + A^a_{12}\partial_{xx}u \\
        \label{eq:acoustic_limit_velocity}
        \partial_t u    + a\partial_x \phi & = A^a_{21}\partial_{xx}\phi + A^a_{22}\partial_{xx}u
    \end{align}
\end{subequations}
which are the equations governing linear acoustics at low Mach number (see Muller ** for more details).
For the artificial diffusion terms to appear in the limit equations, the coefficients should be:
\begin{equation} \label{eq:acoustic_diffusion_scaling}
    \underline{\underline{A}}^a \sim \mathcal{O}
    \begin{matrix}
    \begin{pmatrix}
    M^{-1} & M^{-1} \\
    M^{-1} & M^{-1} \\
    \end{pmatrix}
    \end{matrix}
\end{equation}
We can see that at the acoustic limit, all coefficients of the artificial diffusion scale at the same rate, which is how standard upwind schemes for compressible flow scale at low Mach number.
The diagonal diffusion coefficients for the convective (\ref{eq:convective_diffusion_scaling}) and acoustic (\ref{eq:acoustic_diffusion_scaling}) components have different orders, which is problematic if we are to design a numerical scheme for the two-timescale limit.
We will show why by working out the limit equations assuming the flow variables scale with the convective component but the artificial diffusion scales with the acoustic component, and vice versa.
For convective flow scaling (\ref{eq:symmetric_convective_scaling}) but acoustic diffusion scaling (\ref{eq:acoustic_diffusion_scaling}), the limit equations are:
\begin{subequations} \label{eq:convective_limit_acoustic_diffusion}
    \begin{align}
        \label{eq:pressure_clim_adiff}
        \partial_t \phi                    + a\partial_x u & =                           A^a_{12}\partial_{xx}u \\
        \label{eq:velocity_clim_adiff}
        \partial_t u                                       & =                           A^a_{22}\partial_{xx}u
    \end{align}
\end{subequations}
While for acoustic flow scaling (\ref{eq:symmetric_acoustic_scaling}) but convective diffusion scaling (\ref{eq:convective_diffusion_scaling}), the limit equations are:
\begin{subequations} \label{eq:acoustic_limit_convective_diffusion}
    \begin{align}
        \label{eq:pressure_alim_cdiff}
        \partial_t \phi                                      = A^c_{11}\partial_{xx}\phi                        \\
        \label{eq:velocity_alim_cdiff}
        \partial_t u    + a\partial_x \phi                   = A^c_{21}\partial_{xx}\phi
    \end{align}
\end{subequations}

The acoustic velocity diffusion $A^a_{22}$ and the convective pressure diffusion $A^c_{11}$ are too large for flows at the opposite limit, and turn the limit equations (\ref{eq:velocity_clim_adiff}) and (\ref{eq:pressure_alim_cdiff}) into Poisson/elliptic type equations (depending on if a steady or unsteady solution is sought).
Overdamping of the velocity field (\ref{eq:velocity_clim_adiff}) is a well-known problem with using conventional compressible schemes at low Mach number.
Overdamping of the pressure field (\ref{eq:pressure_alim_cdiff}) will effectively filter out acoustics from the solution - a desired effect if we want solutions at the convective limit, but very undesirable if we want solutions at the two timescale limit.

On the other hand, the acoustic pressure diffusion $A^a_{11}$ and the convective velocity diffusion $A^c_{22}$ are too small for flows at the opposite limit, and disappear from the limit equations (\ref{eq:pressure_clim_adiff}) and (\ref{eq:velocity_alim_cdiff}), leaving only the off-diagonal artificial diffusion components.
Whilst this may provide enough stabilisation in some circumstances, problems may occur when the diagonal field ($\phi$ in (\ref{eq:pressure_clim_adiff}) and $u$ in (\ref{eq:velocity_alim_cdiff})) is oscillatory but the off-diagonal field ($u$ in (\ref{eq:pressure_clim_adiff}) and $\phi$ in (\ref{eq:velocity_alim_cdiff})) is smooth, in which case not enough diffusion will be generated to prevent instabilities.
In the pathological case that either $A^a_{12},A^c_{21} \lesssim \mathcal{O}(M^{-1})$, then the off-diagonal terms will also disappear from the limit equations, leaving no diffusion on either/both of the convective component of pressure (\ref{eq:pressure_clim_adiff}) or the acoustic component of velocity (\ref{eq:velocity_alim_cdiff}).

\textit{Sentence or two here saying what we want from a numerical scheme for the two-timescale limit: limit equations with all the lhs terms from (\ref{eq:convective_limit_equations}) and (\ref{eq:acoustic_limit_equations}), and non-vanishing diffusion on all field.}\\
To create a diffusion matrix suitable for the two timescale limit, we take the lowest order or either $\underline{\underline{A}}^c$ or $\underline{\underline{A}}^a$ for each component:
\begin{equation} \label{eq:blended_diffusion_scaling}
    \underline{\underline{A}}^b \sim \mathcal{O}
    \begin{matrix}
    \begin{pmatrix}
    M^{-1} & M^{-1} \\
    M^{-1} & M^{0} \\
    \end{pmatrix}
    \end{matrix}
\end{equation}
This will allow both convective and acoustic components of pressure and velocity, albeit at the risk of the convective pressure and the acoustic velocity having non-diagonal or vanishing diffusion.
We shall see later that most modern schemes use this scaling, which we shall refer to as the blended scheme, following Sachdev2012**.
While this scaling is widely used, to the authors knowledge Sachdev et al is one of the only papers to explicitly identify the use of acoustic scaling for the pressure and convective scaling for the velocity. They also numerically demonstrate the issue of vanishing diffusion on the convective pressure and acoustic velocity.

The limit equations for convective flow scaling and blended diffusion scaling are:
\begin{subequations} \label{eq:convective_limit_blended_diffusion}
    \begin{align}
        \label{eq:pressure_clim_bdiff}
        \partial_t \phi                    + a\partial_x u & = \phantom{A^b_{21}\partial_{xx}\phi +\,} A^b_{12}\partial_{xx}u \\
        \label{eq:velocity_clim_bdiff}
        \partial_t u    + a\partial_x \phi + u\partial_x u & = A^b_{21}\partial_{xx}\phi + A^b_{22}\partial_{xx}u
    \end{align}
\end{subequations}
The limit equations for acoustic flow scaling and blended diffusion scaling are:
\begin{subequations} \label{eq:acoustic_limit_blended_diffusion}
    \begin{align}
        \label{eq:pressure_alim_bdiff}
        \partial_t \phi + a\partial_x u    & = A^b_{11}\partial_{xx}\phi + A^b_{12}\partial_{xx}u \\
        \label{eq:velocity_alim_bdiff}
        \partial_t u    + a\partial_x \phi & = A^b_{21}\partial_{xx}\phi                          
    \end{align}
\end{subequations}
From which we see that, compared to the desired limit equations (\ref{eq:convective_limit_equations}) and (\ref{eq:acoustic_limit_equations}), all terms on the left-hand sides are present in (\ref{eq:convective_limit_blended_diffusion}) and (\ref{eq:acoustic_limit_blended_diffusion}), so all relevant flow variations can be admitted in the solution.
As stated above, the main limitations of the blended scheme is the vanishing diagonal diffusion terms on the convective pressure and the acoustic velocity, both of which will be explored with numerical examples later.

\subsubsection{Adaptive schemes}

We have identified three possible diffusion matrices - convective, acoustic, and blended - each suited to different flows.
However, it would be useful to have a single numerical method that could select the most appropriate scaling on the fly.
This would be useful either so the same method can be used for multiple problems, or because different flow regimes exist in a single problem \textit{** example from Sachdev?? Helicopter landing?? **}
The major difference between the different schemes is whether they allow acoustic solutions, so a sensible metric for which scheme to use would be whether acoustic waves can actually be resolved by a simulation.
This can be estimated by the ratio of the acoustic timescale $\tau$ and the simulation timestep $\Delta t$:
\begin{equation} \label{eq:unsteady_mach}
    \frac{\tau}{\Delta t} = \frac{L_{\infty}/a}{\Delta t} = \frac{L_{\infty}/\Delta t}{a} = M_u
\end{equation}
When $\Delta t > \tau$, acoustic waves cannot be temporally resolved, and $M_u$ is small.
When $\Delta t < \tau$, acoustic waves can be resolved, and $M_u$ is large.
In practice, $M_u$ is clamped $M$ and $1$ so $M_u\to M$ as $\Delta t\to0$.
If $A_{11}\sim\mathcal{O}(M^{-1}M_u^{-1})$ then the pressure diffusion will range from the convective scaling if $M_u$ is small to the acoustic scaling if $M_u=1$.
Equivalently, $A_{22}\sim\mathcal{O}(M^{-1}M_u)$ can be used to force the velocity diffusion to scale between the convective and acoustic scaling.

The parameter $\tau/\Delta t$ is normally presented as the unsteady Mach number $M_u$, so called because it can be arranged as a "speed" $L_{\infty}/\Delta t$ divided by $a$.
To the author's knowledge, this parameter was first introduced by Venkateswaran \& Merkle **1995** to improve the conditioning of the inner iterations of a preconditioned dual-time scheme.
The use of $M_u$ in preconditioned schemes is equivalent to its use in both $A_{11}$ and $A_{22}$, so the numerical method varies from the fully convective scheme to the fully acoustic scheme.
Venkateswaran and Merkle later identified that returning fully to the acoustic limit created undesirably high diffusion on the velocity field \textit{**Evaluation of artificial dissipation models and their relationship to the accuracy of Euler and Navier-Stokes computations**}.
Sachdev et al's blended preconditioning is essentially designed to resolve this by using $M_u$ for the pressure diffusion $A_{11}$ but not the velocity diffusion $A_{22}$, therefore their schemes (both preconditioned FDS and AUSM) vary between the fully convective scheme and the blended scheme.

\subsubsection{Spectral radius of low Mach number schemes}
We now estimate the growth of the spectral radii of $\underline{\underline{A}}^c$ and $\underline{\underline{A}}^a$ as $M\to0$.
The maximum spectral radius of the convective and diffusive flux components in a numerical scheme determines the CFL bound required for stability in an explicit timestepping scheme, and also affects the convergence behaviour of implicit schemes through the condition number.
The spectral radius of the physical flux Jacobian, $u+a$, grows as $\mathcal{O}(M^{-1})$ in the limit $M\to0$, so if the spectral radius of the artificial diffusion grows faster than this, it will induce a more stringent stability bound on the numerical scheme.
It can be seen from (\ref{eq:convective_diffusion_scaling}) and (\ref{eq:acoustic_diffusion_scaling}) that the traces of the two coefficient matrices will grow as:
\begin{equation} \label{eq:trace_growths}
    \text{tr}(\underline{\underline{A}}^c) \sim \mathcal{O}(M^{-2}),
    \quad
    \text{tr}(\underline{\underline{A}}^a) \sim \mathcal{O}(M^{-1})
\end{equation}
Given the trace is the sum of the eigenvalues, and is an invariant of the matrix, we can use (\ref{eq:trace_growths}) to estimate the growth of the spectral radii\footnote[2]{
    The trace of a matrix can grow more slowly than the spectral radius due to cancellation.
    For example, the trace of the Euler equations flux Jacobian in $N$ dimensions is $(N+2)u$, which is $\mathcal{O}(1)$, even though the spectral radius is $\mathcal{O}(M^{-1})$.
    However, a well designed diffusion matrix is positive-definite, which makes cancellation impossible.
    Additionally, the trace cannot grow faster than the spectral radius for any matrix.
    As the trace of a diffusion matrix cannot grow asymptotically faster or slower than the spectral radius, it is an appropriate estimate for the scaling of the spectral radius.}.
The trace in the acoustic limit grows at the same rate as the physical spectral radius, so it will not change the stability requirements - up to a constant factor.
On the other hand, the trace in the convective limit grows faster than the physical spectral radius by an order of $M$, so will require a CFL bound which decreases one order faster than the physical CFL bound in order to remain stable as $M\to0$.
This scaling in the convective limit was proven by Birken \& Meister for the specific case when the artificial diffusion is due to a flux Jacobian with low Mach number preconditioning **.
However, our estimate implies that this restriction will hold for any scheme whose diffusion converges to the convective limit as $M\to0$.
Later we will see that this is true for existing AUSM schemes that converge to this limit.\\
\textit{\textcolor{red}{What about the Thornber and Rieper fixes? Both of these proved the pressure field has 2nd order variation, but say the spectral radius was unchanged. Should check this. Gu and Li put these fluxes in almost the form that we put AUSM in. See if they increase the pressure flux or only reduce the velocity flux (pressure diffusion drives spectral radius estimate). NOTE: reducing velocity diffusion prevents anomalous creation of acoustic pressure, increase in pressure diffusion damps existing acoustic pressure. Also could put comment here about "instantaneous" divergence-pressure coupling just means faster than any physical wave, and all other schemes for convective limit solve some implicit problem, why should density based be different?}} \\

Finally, before moving on to the next section, we consider the coefficients $A_{33}$ and $A_{44}$ of the artificial diffusion on the linear fields (\ref{eq:vorticity_symmetric}) and (\ref{eq:entropy_symmetric}).
In both limits, the terms on the left hand side of these equations are $\mathcal{O}(v)$ and $\mathcal{O}(s)$ respectively.
The vorticity field is $\mathcal{O}(M^0)$ in both limits, so the coefficient $A_{33}$ should both be $\mathcal{O}(M^0)$ for the artificial diffusion to be well balanced.
The scaling of the entropy field however, depends on the specific case.
Entropy is generated by viscous effects ($\mathcal{O}(1/Re)$) and heat addition, so without knowing how these scale with, or compare to, the Mach number we cannot state the appropriate scaling for $A_{44}$, other than to assume that $\mathcal{O}(M^0)$ might be a good starting point, purely from examination of the physical flux Jacobian.
\textit{\textcolor{red}{Entropy generation is due to source terms, which are not included in our formulation}}.
For a discussion of the effects of viscosity and heat addition at low Mach number, see the VKI lectures by Muller ** and references therein.

==> sections/ausm_comparison.tex <==
Work out Jacobian coefficients for each AUSM flux
\begin{itemize}
    \item contribution of Van Leer Mach/pressure splitting to interface velocity/pressure diffusion
    \item contribution of additional diffusion terms to Jacobian
    \item analyse: AUSM+up, LDFSS2001, SLAU, SLAU-WS, AUSM+up'
    \item for each flux:
    \begin{itemize}
        \item convective or acoustic asymptotic behaviour (or neither?)
        \item collateral diffusion from enforcing correct scaling at low mach
        \item spectral radius
    \end{itemize}
    \item compare fluxes with the same asymptotic behaviour (LSDF2001 / AUSM+up, SLAU-AS / AUSM+up')
    \item analyse existing diffusion reduction strategies: (flux2 \& HR-flux)
\end{itemize}

\subsection{LDFSS2001}
\textit{Convective limit found from analogy to preconditioned system}\\

\subsection{AUSM$^+$-up}
\textit{Convective limit found from discrete asymptotic analysis}\\
AUSM$^+$-up was designed by Liou in 2006 to combine the success of pressure-velocity coupling terms of previous AUSM fluxes with the low Mach number capabilities of LDFSS2001 **.
Liou considered only the convective low Mach limit, and used a discrete asymptotic analysis to rigorously derive the required scaling of the diffusion terms as $M\to0$.
At low Mach number, the interface velocity and pressure in AUSM$^+$+up are (Appendix **):
\begin{equation} \label{eq:ausmpup:interface_velocity_lm}
    u_{1/2} = \{u\} - \frac{\llbracket p \rrbracket}{8\rho a \overline{M}} + \mathcal{O}(M^3)
\end{equation}
\begin{equation} \label{eq:ausmpup:interface_pressure_lm}
    p_{1/2} \approx \{p\} - \bigg( \frac{3\rho a \overline{M}}{8} + \frac{15\rho a M^2}{4} \bigg)\llbracket u \rrbracket + \mathcal{O}(M^4)
\end{equation}
Where $\overline{M}$ is the local Mach number clamped between a lower cutoff $M_{co}$ and 1.
The lower cutoff prevents division by zero in (\ref{eq:ausmpup:interface_velocity_lm}), and the upper limit ensures the low Mach number scaling does not affect the scheme in supersonic flow.
\begin{equation} \label{eq:mach_number_clamped}
    \overline{M} = \texttt{min}(1,\texttt{max}(M,M_{co}))
\end{equation}
From (\ref{eq:ausmpup:interface_velocity_lm}) and (\ref{eq:ausmpup:interface_pressure_lm}) it can be see that:
\begin{equation} \label{eq:ausmpup_nu_convective}
    \nu_u \approx 0,
    \quad
    \nu_p = \frac{1}{8\rho a M} \sim \mathcal{O}(M^0)
\end{equation}
\begin{equation} \label{eq:ausmpup_mu_convective}
    \mu_p \approx 0,
    \quad
    \mu_u \approx -\frac{3\rho a M}{8} \sim \mathcal{O}(M^0)
\end{equation}
Where the second term in brackets in (\ref{eq:ausmpup:interface_pressure_lm}) is an order of $M$ smaller than the first, so has been neglected.
Collecting (\ref{eq:ausmpup_nu_convective}) and (\ref{eq:ausmpup_mu_convective}) together, the diffusion matrix of AUSM$^+$-up scales as:
\begin{equation} \label{eq:ausmpup_scaling_convective}
    \underline{\underline{A}} \sim \mathcal{O}
    \begin{matrix}
    \begin{pmatrix}
        M^{-2} & 0     \\
        0      & M^{0} \\
    \end{pmatrix}
    \end{matrix}
\end{equation}
This is a diagonal approximation to the convective limit diffusion matrix (\ref{eq:convective_diffusion_scaling}).
This result is unsurprising given the use of a discrete asymptotic analysis in the derivation of AUSM$^+$-up, and almost 15 years of evidence of AUSM$^+$-up producing satisfactory results for convective low Mach number problems, however it again verifies the correctness of our method.

In the original paper, Liou recognised that the asymptotic analysis relies on the assumptions of a uniform background pressure and that a convective limit solution is sought, and recommended that for situations where these assumptions do not hold, the low Mach number scaling factor $f_a$ should be fixed equal to one.
In this case, the diagonal coefficients $\nu_p$ and $\mu_u$ decrease and increase by an order of $M$ respectively, and the approximation $\alpha\approx-\frac{3}{4}$ in the pressure splitting is no longer valid.
The resulting diffusion coefficients are:
\begin{equation} \label{eq:ausmpup_nu_acoustic}
    \nu_u \approx 0,
    \quad
    \nu_p = \frac{1}{4\rho a} \sim \mathcal{O}(M^1)
\end{equation}
\begin{equation} \label{eq:ausmpup_mu_acoustic}
    \mu_p \approx 0,
    \quad
    \mu_p \approx -\frac{21\rho a}{16} \sim \mathcal{O}(M^{-1})
\end{equation}
and the diffusion matrix scales now as:
\begin{equation} \label{eq:ausmpup_scaling_acoustic}
    \underline{\underline{A}} \sim \mathcal{O}
    \begin{matrix}
    \begin{pmatrix}
        M^{-1} & 0      \\
        0      & M^{-1} \\
    \end{pmatrix}
    \end{matrix}
\end{equation}
Which is a diagonal approximation of the acoustic limit diffusion matrix (\ref{eq:acoustic_diffusion_scaling}), showing that with $f_a=1$, AUSM$^+-up$ is suitable for low Mach number acoustic problems.

\subsection{AUSM$^+$up' \& AUSM$^+$u'p'}
\textit{use timestep ratio to decide $f_a$ for pressure diffusion on mass flux and velocity diffusion on pressure - changes $A_{11}$, $A_{12}$ and $A_{22}$ elements of Jacobian.}\\
Sachdev et al ** investigated preconditioned Roe and AUSM type fluxes for low Mach numbers, specifically flow with both convective and acoustic phenomena.
They pointed out that the large pressure diffusion in convective schemes (\ref{eq:convective_diffusion_scaling}) quickly damps acoustic waves, while the large velocity diffusion in acoustic schemes (\ref{eq:acoustic_diffusion_scaling}) severely damps convective phenomena such as vortices.
Neither form is therefore suitable for flows where convective and acoustic phenomena coexist and interact.
They formulate a 'blended' preconditioning for flux-difference splitting schemes which takes the pressure diffusion from the acoustic matrix and the velocty diffusion from the convective matrix - i.e. the smallest diffusion on each field.
This blended scheme gave improved results over a range of problems, with one exception being a low Mach number shock tube problem we will study later.
To control this blending, they include an 'unsteady Mach number' $M_u$, in the choices for the preconditioning parameter $\beta$, which is the same as $\overline{M}$ in (\ref{eq:mach_number_clamped}).
\begin{equation} \label{eq:unsteady_mach_number}
    M_u = \frac{L}{\pi a \Delta t},
\end{equation}
This definition of $M_u$ was first used by Venkateswaran \& Merkle **, who derived it as a way of improving the condition number of preconditioned dual-timestepping schemes with very small timesteps at low Mach number.g in the bac
It is commonly called an unsteady Mach number because of its use in (\ref{eq:preconditioning_parameter}) with the local and cutoff (and sometime viscous **Weiss \& Smith) Mach numbers.
However, $L/a=\tau$ is the acoustic timescale used for the two-timescale asymptotic analysis in section **, meaning that $M_u$ can also be thought of as a ratio of timescales $\tau/\Delta t$ (except for a factor of $1/\pi$ which is a result of the Fourier analysis approach of V\&M).
$M_u$ says that if $\Delta t > \tau$, the acoustic timescale is unresolved, so the convective limit scheme should be used, whereas if $\Delta t < \tau$, the acoustic timescale is resolved, so the acoustic limit scheme should be used.
Sachdev et al extend the blended preconditioning approach to AUSM$^+$-up by using (\ref{eq:unsteady_mach_number}) in the calculation of the pressure diffusion in the interface velocity (\ref{eq:ausmpup:interface_velocity_lm}). For small timesteps $M_u=1$ and the pressure diffusion is decreased by an order of $M$, becoming equivalent to the acoustic scaling (\ref{eq:ausmpup_mu_acoustic}).
The diffusion matrix of this scheme - called AUSM$^+$-up' because of the modification to the pressure diffusion - scales as:
\begin{equation} \label{eq:ausmpup'_scaling_acoustic}
    \underline{\underline{A}} \sim \mathcal{O}
    \begin{matrix}
    \begin{pmatrix}
        M^{-1} & 0     \\
        0      & M^{0} \\
    \end{pmatrix}
    \end{matrix}
\end{equation}
Where we can see that the pressure field is damped according to the acoustic scaling, and the velocity field is damped according to the convective scaling - the lowest choice for each field.
This scheme performed well for almost all test cases, and in some cases outperformed the blended preconditioning flux-difference scheme.
They both failed for a low Mach shocktube case, however a solution was proposed, where $M_u$ is used in the calculation of both the velocity and pressure diffusion terms.
For small timesteps, this scheme, called AUSM$^+$-u'p', reverts to AUSM$^+$-up without the low Mach number scaling, whose diffusion matrix was shown in (\ref{eq:ausmpup_scaling_acoustic}) - i.e. the scheme suggested by Liou for shock tube problems.
The benefit of AUSM$^+$-up' and AUSM$^+$-u'p' is that they locally adapt between different scalings, so can be used in simulations where both very high and low speed flow exist simulataneously, or between different simulations with different requirements without modification.

\subsection{SLAU}
\textit{Acoustic limit found from SHUS mass flux and "reducing" dissipation compared to AUSM+-up}\\

\subsection{SLAU-WS}
\textit{Very ad-hoc solution to alter diffusive terms based on a pressure "wiggle-sensor". When switched on, wiggle sensor returns convective scaling?}\\

\subsection{AUSM-M}
\textit{Acoustic limit from following SLAU on "reduced" mass flux dissipation and some AUSMPW+ base}\\

\subsection{A minimal AUSM scheme for either limit}
\textit{AUSM scheme with absolutely minimal possible diffusive terms and adaptive to both limits}\\

\subsection{Reduced diffusion at convective limit}
\textit{What has lower diffusion - AUSM+up, LDSF2001, SLAU-AS (at large dt)? How do hr-flux and flux2 modifications change this?}\\

\subsection{Reduced diffusion at acoustic limit}
\textit{What has lower diffusion - SLAU, AUSM+up', AUSM+u'p' (both at large dt)? How do hr-flux and flux2 modifications change this?}\\

==> sections/ausm_fds_recasting.tex <==
Recast AUSM family of fluxes as flux difference splitting scheme to isolate the diffusive flux Jacobian.
\begin{itemize}
    \item immediate form of flux Jacobian - fluxes in conserved variables, jumps in u,p and convected variables
    \item transform to symmetry variables
    \item show it doesn't matter (for us) if you define AUSM with interface velocity or interface mass flow
    \item analysis of general ausm flux Jacobian
    \begin{itemize}
        \item which AUSM parameters affect which fields?
        \item which AUSM parameters decide the scaling necessary for low mach asymptotes?
        \item coupling of linear to nonlinear fields / vice-versa?
        \item any other obvious simplifications or desirable features?
        \item general expressions for eigenvalues of ausm fluxes
    \end{itemize}
\end{itemize}

\subsection{Flux formulations}
We briefly describe the formulation of AUSM schemes and flux-difference splitting schemes, as preparation for transforming AUSM into an equivalent flux-difference splitting form.
\subsubsection{AUSM family fluxes}
The AUSM family of fluxes have the following general form:
\begin{equation} \label{eq:ausm_form}
    \underline{\hat{f}} =  \frac{u_{1/2} + |u_{1/2}|}{2}\underline{\varphi}_{L}
                         + \frac{u_{1/2} - |u_{1/2}|}{2}\underline{\varphi}_{R}
                         + p_{1/2}\underline{N}
\end{equation}
\begin{equation}
\underline{\varphi} = 
    \begin{matrix}
    \begin{pmatrix}
        \rho \\ \rho u \\ \rho v \\ \rho h
    \end{pmatrix}
    \end{matrix},
    \quad
    \quad
\underline{N} = 
    \begin{matrix}
    \begin{pmatrix}
        0 \\ n_x \\ n_y \\ 0
    \end{pmatrix}
    \end{matrix}
\end{equation}
where underlining indicates vector valued quantities, $\underline{\hat{f}}$ is the interface flux, $\underline{\varphi}$ is the vector of convected quantities, $\underline{N}$ is the (zero padded) interface normal vector, and $u_{1/2}$ and  $p_{1/2}$ are interface velocity and pressure respectively.
A specific AUSM scheme is uniquely determined by the definition of interface velocity and pressure.
Note that this form differs slightly from the usual presentation, where the interface velocity is replaced by an interface mass flow $\dot{m}_{1/2}$, and $\underline{\varphi}=(1, u, v, h)$ in equation (\ref{eq:ausm_form}).
However, usually the interface mass flow is defined as:
\begin{equation} \label{eq:interface_mass_flow}
    \dot{m}_{1/2} = u_{1/2}
    \begin{cases}
        \rho_L, & \text{if}\ u_{1/2} > 0 \\
        \rho_R, & \text{otherwise}
    \end{cases}
\end{equation}
making the two forms equivalent.
One notable exception is SLAU **, where the interface mass flow is not calculated using equation (\ref{eq:interface_mass_flow}).
However, they show in their paper (equations (24b) and (24c)) that the interface mass flux function of SLAU reduces to (\ref{eq:interface_mass_flow}) if both the left and right velocities are of the same sign.
As we expect this to be the case at most cell interfaces, we will use this simplification when we consider SLAU later in the paper.
We show the conditions which must hold to make this simplification more generally in Appendix **.

\subsubsection{Flux difference splitting fluxes}
Flux difference splitting (FDS) schemes have the following general form:
\begin{equation} \label{eq:fds_form}
    \underline{\hat{f}} = \{\underline{f}\} - \frac{|\underline{\underline{A}}|}{2} \llbracket \underline{q} \rrbracket
\end{equation}
where $\{(\cdot)\} = \frac{(\cdot)_L + (\cdot)_R}{2}$ is the arithmetic average and $\llbracket (\cdot) \rrbracket = (\cdot)_R - (\cdot)_L$ is the jump over an interface. $\underline{f}$ is the exact inviscid flux function, $|\underline{\underline{A}}|$ is the diffusive flux Jacobian where $|(\cdot)|$ indicates positive (semi-)definiteness, and $\underline{q}$ is the vector of state variables.
The diffusive flux Jacobian $|\underline{\underline{A}}|$ uniquely determines an FDS scheme.
The FDS form is useful because it distinguishes between the non-diffusive central part of the flux $\{\underline{f}\}$, and the diffusive upwind correction $|\underline{\underline{A}}| \llbracket \underline{q} \rrbracket$.
If the diffusive flux Jacobian is in symmetrising form, we can make direct comparison to the artificial diffusion in equation (\ref{eq:euler_symmetric}), and make use of the results of the previous section for numerical schemes at low Mach number.

\subsection{AUSM fluxes in FDS form}
The $\frac{u_{1/2} \pm |u_{1/2}|}{2}$ coefficients in equation (\ref{eq:ausm_form}) simply act as a switch to upwind the convected variables $\underline{\varphi}$ so, without loss of generality, we assume $u_{1/2} > 0$ and reduce equation (\ref{eq:ausm_form}) to:
\begin{equation} \label{eq:ausm_form2}
    \underline{\hat{f}} = u_{1/2}\underline{\varphi}_L + p_{1/2}\underline{N}
\end{equation}
To rewrite equation (\ref{eq:ausm_form2}) in FDS form (equation (\ref{eq:fds_form})), we write the interface velocity and pressure as a central approximation plus some diffusive terms:
\begin{equation} \label{eq:interface_up}
    \begin{split}
        u_{1/2} & = \{u\} - u_d \\
        p_{1/2} & = \{p\} - p_d
    \end{split}
\end{equation}
By adding $\big(u_R\underline{\varphi}_R - u_R\underline{\varphi}_R\big)/2$ to the right hand side of equation (\ref{eq:ausm_form2}) and rearranging, we find:
\begin{equation} \label{eq:ausm_form3}
    \underline{\hat{f}} = \{\underline{f}\} - \frac{u_R}{2}\llbracket\underline{\varphi}\rrbracket - u_d\underline{\varphi}_L - p_d\underline{N}
\end{equation}
where we see the interface flux is now composed of a central approximation plus some diffusive terms.
For most AUSM fluxes, the diffusive terms of the interface velocity and pressure are functions only of the jumps in the pressure and face normal velocity, so $u_d$ and $p_d$ can be written as:
\begin{equation} \label{eq:interface_up_diffusion}
    \begin{split}
        u_d & = \nu_p \llbracket p \rrbracket + \nu_u \llbracket u \rrbracket \\
        p_d & = \mu_p \llbracket p \rrbracket + \mu_u \llbracket u \rrbracket
    \end{split}
\end{equation}
We can now write the diffusive terms of equation \ref{eq:ausm_form3} as:\\
\textit{\textcolor{red}{The velocity and pressure diffusion terms in this equation and the next can be written as matrices or as Cartesian products between two vectors. Which is better? The matrix form is more standard, but I like the Cartesian product form as it clearly shows the structure, and that these terms are rank-deficient (is the rank-deficiency even important? Does the rank deficiency show that there exists a basis where each term only affects one field, which would be useful?)}}
\begin{equation} \label{eq:ausm_diffusion_immediate}
    u\underline{\underline{I}}
    \begin{matrix}
        \begin{pmatrix}
            \llbracket \rho  \rrbracket \\
            \llbracket \rho u\rrbracket \\
            \llbracket \rho v\rrbracket \\
            \llbracket \rho h\rrbracket
        \end{pmatrix}
    \end{matrix}
    +
    \Bigg[
    \begin{matrix}
        \begin{pmatrix}
            \nu_p \rho    & \nu_u \rho   \\
            \nu_p \rho u  & \nu_u \rho u \\
            \nu_p \rho v  & \nu_u \rho v \\
            \nu_p \rho u  & \nu_u \rho h
        \end{pmatrix}
    \end{matrix}
    +
    \begin{matrix}
        \begin{pmatrix}
            0     & 0 \\
            \mu_p & \mu_u \\
            0     & 0 \\
            0     & 0
        \end{pmatrix}
    \end{matrix}
    \Bigg]
    \begin{matrix}
        \begin{pmatrix}
            \llbracket p \rrbracket \\
            \llbracket u \rrbracket
        \end{pmatrix}
    \end{matrix}
\end{equation}

\begin{equation}
    u\underline{\underline{I}}
    \begin{matrix}
        \begin{pmatrix}
            \llbracket \rho  \rrbracket \\
            \llbracket \rho u\rrbracket \\
            \llbracket \rho v\rrbracket \\
            \llbracket \rho h\rrbracket
        \end{pmatrix}
    \end{matrix}
    +
    \Bigg[
    \begin{matrix}
        \begin{pmatrix}
            \rho   \\
            \rho u \\
            \rho v \\
            \rho h 
        \end{pmatrix}
        \begin{pmatrix}
            \nu_p & \nu_u
        \end{pmatrix}
    \end{matrix}
    +
    \begin{matrix}
        \begin{pmatrix}
            0 \\
            1 \\
            0 \\
            0 
        \end{pmatrix}
        \begin{pmatrix}
            \mu_p & \mu_u
        \end{pmatrix}
    \end{matrix}
    \Bigg]
    \begin{matrix}
        \begin{pmatrix}
            \llbracket p \rrbracket \\
            \llbracket u \rrbracket
        \end{pmatrix}
    \end{matrix}
\end{equation}

Where we have rotated the coordinate system to be aligned with the interface so that the pressure flux appears only in the normal momentum equation, and dropped the $L/R$ subscripts on the state variables.
At low Mach number the flow should be smooth, meaning the relative difference between left and right states will be small.
As we are interested in general behaviour and scaling, this simplification should not be of consequence.
The first term in equation (\ref{eq:ausm_diffusion_immediate}) is due to the upwinding of the convected variables, while the second and third terms are due to the diffusive contributions to the interface velocity and pressure respectively.

We transform equation (\ref{eq:ausm_diffusion_immediate}) to entropy variables by pre-multiplying every term by the Jacobian matrix $\frac{\partial \underline{q}^s}{\partial \underline{q}^c}$, substituting $\llbracket \underline{\varphi} \rrbracket = \frac{\partial \underline{\varphi}}{\partial \underline{q}^s} \llbracket \underline{q}^s \rrbracket$ in the upwinding term, and substituting $\llbracket p \rrbracket = \rho a \llbracket \phi \rrbracket$ in the last two terms (see Appendix **).
After these manipulations, equation (\ref{eq:ausm_diffusion_immediate}) becomes:
\begin{equation} \label{eq:ausm_diffusion_symmetric}
    \Bigg[
    u
    \begin{matrix}
        \begin{pmatrix}
            \gamma & 0 & 0 & 0 \\
            0      & 1 & 0 & 0 \\
            0      & 0 & 1 & 0 \\
            \Gamma & 0 & 0 & 1
        \end{pmatrix}
    \end{matrix}
    + 
    \begin{matrix}
        \begin{pmatrix}
            1 \\
            0 \\
            0 \\
            0 
        \end{pmatrix}
        \begin{pmatrix}
            \rho a^2\nu_p & a\nu_u & 0 & 0
        \end{pmatrix} \\
    \end{matrix}
    +
    \begin{matrix}
        \begin{pmatrix}
            -\Gamma u/a \\
            1 \\
            0 \\
            -\Gamma u/a \\
        \end{pmatrix}
        \begin{pmatrix}
            a\mu_p & \mu_u/\rho & 0 & 0
        \end{pmatrix} \\
    \end{matrix}
    \Bigg]
    \begin{matrix}
        \begin{pmatrix}
            \llbracket \phi  \rrbracket \\
            \llbracket u     \rrbracket \\
            \llbracket v     \rrbracket \\
            \llbracket \zeta \rrbracket
        \end{pmatrix}
    \end{matrix}
\end{equation}

where $\Gamma=\gamma-1$.
First we look at the upwinding contribution.
The velocity and vorticity are upwinded by the correct magnitude ($u$), and are not affected by jumps in other variables in this term.
However, the pressure is over-upwinded by a factor of $\gamma$, and the entropy is erroneously upwinded by jumps in the pressure, which introduces coupling between the linear and acoustic subsystems which is not present in the physical flux Jacobian (\ref{eq:symmetric_jacobian}).
These "imperfections" in the upwinding are because, in the standard AUSM form (\ref{eq:ausm_form}), the upwinding is on the convected variables $\underline{\varphi}$ but fluxes are calculated in the conserved variables $\underline{q}^c$.
As a result, the matrix multiplying $u$ in the upwinding is equal to $\frac{\partial \underline{q}^s}{\partial \underline{q}^c} \frac{\partial \underline{\varphi}}{\partial \underline{q}^s}$.

The second term in (\ref{eq:ausm_diffusion_symmetric}), from the diffusive terms in the interface velocity, affects only the pressure equation.
This will prove useful later when we estimate the required scaling of these terms, as we can make these estimates based only on requirements on the pressure field, without affecting any other field.

Finally, we have the contribution from the diffusive terms in the interface pressure.
This provides diffusion only on the velocity field which, like for the interface velocity diffusion, we will use later to estimate the required scaling of these terms.
However, the diffusion on the interface pressure also results in anti-diffusion terms in the pressure and entropy equations, which can be seen from the $-\Gamma u/a$ terms with negative sign.
This is problematic only if these anti-diffusion terms do not disappear in the limit equations, i.e. if they are the same order of $M$, or lower, than the largest term in the pressure or entropy equations.
The anti-diffusion on the entropy from the interface pressure diffusion introduces additional coupling between the acoustic subsystem and the entropy field, on top of the coupling caused by the erroneous upwinding of the entropy by jumps in the pressure.

We now write out the diffusion on each equation separately: \\
\begin{subequations}
Symmetric pressure $\phi$:
\begin{equation}
    \big(u(\mu_p + \gamma(1 - \mu_p)) + \rho a^2 \nu_p \big) \llbracket \phi \rrbracket + 
    \big(a\nu_u -   \frac{(\gamma-1)u}{\rho a}\mu_u \big)   \llbracket u    \rrbracket
    \label{eq:sym_pressure_diffusion}
\end{equation}
Velocity $u$:
\begin{equation}
    a\mu_p\big                       \llbracket \phi \rrbracket + 
    \big(u + \frac{\mu_u}{\rho}\big) \llbracket u \rrbracket
    \label{eq:sym_velocity_diffusion}
\end{equation}
Vorticity $v$:
\begin{equation}
    u \llbracket v \rrbracket
    \label{eq:sym_vorticity_diffusion}
\end{equation}
Symmetric entropy $\zeta$:
\begin{equation}
    u(\gamma-1)(1-\mu_p)              \llbracket \phi \rrbracket - 
    \frac{(\gamma-1)u}{\rho a}\mu_u   \llbracket u    \rrbracket +
    u                                 \llbracket \zeta \rrbracket
    \label{eq:sym_entropy_diffusion}
\end{equation}
\end{subequations}

In the pressure and velocity equations, we see that $\nu_p$, $\nu_u$, $\mu_p$ and $\mu_u$ provide dissipation in the $A_{11}$, $A_{12}$, $A_{21}$, $A_{22}$ terms respectively, which will be used shortly to derive the required scaling of these coefficients to achieve accurate solutions in the convective or acoustic limits as $M\to0$.
We can also see the negative diffusion in the pressure equation with $\mu_p$ and $\mu_u$ as previously noted.
The terms $\nu_p$ and $\mu_u$ are often called the pressure-velocity coupling, as they add pressure diffusion to the interface velocity, and velocity diffusion to the interface pressure respectively.
We can see from (\ref{eq:sym_pressure_diffusion}) and (\ref{eq:sym_velocity_diffusion}) however that the role they play in the symmetrised variable form is to provide diffusion on the pressure field with jumps in the pressure, and diffusion on the velocity field with jumps in the velocity, which will help damp oscillations in these fields.

Interestingly, the diffusion on the vorticity equation is "ideal", in the sense that it reduces exactly to an upwinding with the scale of the local velocity, with no coupling to any other fields, which mirrors exactly the form of the physical flux Jacobian.
The upwinding on the entropy also scales with the local velocity, but as noted previously, there are some erroneous terms which couple the entropy to the acoustic subsystem.

\subsubsection{Requirements on the interface pressure and velocity diffusion}
\textit{Work out how $\nu_p$, $\nu_u$, $\mu_p$ and $\mu_u$ need to scale for the $A_{ij}$ coefficients to scale correctly in the convective and acoustic limits. Is there any freedom for choices or are you fully constrained?}

We determine the required scaling of the AUSM parameters $\nu_p$, $\nu_u$, $\mu_p$ and $\mu_u$ by comparing the scaling of the artificial dissipation coefficients (\ref{eq:convective_diffusion_scaling}) and (\ref{eq:acoustic_diffusion_scaling}) with the diffusion terms (\ref{eq:sym_pressure_diffusion}) and (\ref{eq:sym_velocity_diffusion}).
First, we consider the off-diagonal terms $A_{12}$ and $A_{21}$, as these have the same scaling $\mathcal{O}(M^{-1})$ at both the convective and acoustic limits.
Using $a\sim\mathcal{O}(M^{-1})$ and ignoring anti-diffusion terms, we find:
\begin{equation}
    A_{12} \sim \mathcal{O}(\nu_u M^{-1}),
    \quad
    A_{21} \sim \mathcal{O}(\mu_p M^{-1})
\end{equation}
So for correct solutions at either limit, we must have:
\begin{equation} \label{eq:offdiagonal_ausm_scaling}
    \nu_u \sim \mathcal{O}(M^0),
    \quad
    \mu_p \sim \mathcal{O}(M^0)
\end{equation}
These parameters can be asymptotically smaller, but if so then the off-diagonal terms disappear from the limit equations as $M\to0$.
Next, we look at the diagonal terms $A_{11}$ and $A_{22}$.
Again ignoring anti-diffusive terms, we find:
\begin{equation}
    A_{11} \sim \mathcal{O}(\nu_p M^{-2}),
    \quad
    A_{22} \sim \mathcal{O}(\mu_u M^{0})
\end{equation}
By comparing to the scaling in the convective limit (\ref{eq:convective_diffusion_scaling}), we must have:
\begin{equation} \label{eq:diagonal_ausm_convective_scaling}
    \nu^c_p \sim \mathcal{O}(M^0),
    \quad
    \mu^c_u \sim \mathcal{O}(M^0)
\end{equation}
and comparing to the scaling in the acoustic limit (\ref{eq:acoustic_diffusion_scaling}), we must have:
\begin{equation} \label{eq:diagonal_ausm_acoustic_scaling}
    \nu^a_p \sim \mathcal{O}(M^1),
    \quad
    \mu^a_u \sim \mathcal{O}(M^{-1})
\end{equation}
These scaling requirements are summarised in Table \ref{table:ausm_parameter_scaling}.
At the convective limit, all diffusion coefficients must become independent of the Mach number, which makes intuitive sense as in this limit we expect to approach the incompressible solution, where the Mach number loses any real meaning.
At the acoustic limit, the diffusion on the pressure must be decreased to allow a first order variation (compared to the second order variation at the convective limit).
As discussed in section **, the diffusion on the velocity must be increased, because the magnitude of the term $a\partial_x \phi$ on the left hand side of equation (\ref{eq:velocity_symmetric}) increases by an order of $M$ relative to the convective limit.
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|} \hline
             & Convective         & Acoustic              & Blended             \\ \hline
     $\nu_p$ & $\mathcal{O}(M^0)$ & $\mathcal{O}(M^1)$    & $\mathcal{O}(M^1)$  \\ \hline
     $\nu_u$ & $\mathcal{O}(M^0)$ & $\mathcal{O}(M^0)$    & $\mathcal{O}(M^0)$  \\ \hline
     $\mu_p$ & $\mathcal{O}(M^0)$ & $\mathcal{O}(M^0)$    & $\mathcal{O}(M^0)$  \\ \hline
     $\mu_u$ & $\mathcal{O}(M^0)$ & $\mathcal{O}(M^{-1})$ & $\mathcal{O}(M^0)$  \\ \hline
\end{tabular}
\caption{Required scaling of the interface velocity and pressure diffusion coefficients in AUSM schemes to achieve accurate solutions at the convective and acoustic low Mach number limits.}
\label{table:ausm_parameter_scaling}
\end{center}
\end{table}

Now we know the correct scaling of the diffusion coefficients at both limits, we consider the anti-diffusive terms on the pressure (\ref{eq:sym_pressure_diffusion}) and entropy (\ref{eq:sym_entropy_diffusion}) fields.
The anti-diffusive terms on the pressure in the convective limit are:
\begin{equation}
    -\Gamma u \mu_p \sim \mathcal{O}(M^0),
    \quad
    -\frac{\Gamma u}{\rho a} \mu_u \sim \mathcal{O}(M^1)
\end{equation}
and in the acoustic limit:
\begin{equation}
    -\Gamma u \mu_p \sim \mathcal{O}(M^0),
    \quad
    -\frac{\Gamma u}{\rho a} \mu_u \sim \mathcal{O}(M^0)
\end{equation}
Which means that the anti-diffusive terms in the pressure equation are always at least one order of $M$ smaller than the diffusive terms, in both limits, so should not cause any instabilities in the scheme.

\subsubsection{Diffusion on the entropy field}
\textit{The diffusion on entropy has contributions from the acoustic subsystem. This seems less than ideal (especially for combustion, which is something the JAXA guys want to do with SLAU). Can this diffusion be decreased while still conforming to the restrictions for proper scaling? You know what a sound wave looks like (from the acoustic eigenvectors), so you can get an estimate for the eronious diffusion on entropy from a single forward/backward travelling soundwave.}

For the entropy equation, recall that we do not know the scaling of the entropy field unless we have information on the entropy generation mechanisms in a particular case (usually viscous effects and/or heat addition either from an outside source or chemical reaction).
\textit{\textcolor{red}{Small comment on scaling of entropy in last paragraph of section 2.2. Definitely feels like conjecture, would be good to see if there are any proper estimations for entropy scaling, as it's a bit wooly at the moment.}}
Because of this, we consider the entire diffusion terms, not just the coefficients.

\begin{subequations} \label{eq:convective_entropy_diffusion_scaling}
Assuming the coefficients $\mu_p$ and $\mu_u$ have the correct scale, in the convective limit we have for the diffusive terms:
\begin{equation}
    u\Gamma\llbracket\phi\rrbracket \sim \mathcal{O}(M),
    \quad
    u\llbracket\zeta\rrbracket \sim \mathcal{O}(\zeta)
\end{equation}
and the anti-diffusive terms:
\begin{equation}
    -\Gamma u \mu_p \llbracket\phi\rrbracket \sim \mathcal{O}(M),
    \quad
    -\frac{\Gamma u}{\rho a} \mu_u \llbracket u \rrbracket \sim \mathcal{O}(M)
\end{equation}
\end{subequations}
All the unwanted terms (the terms coupling the entropy to the acoustic subsystem) are $\mathcal{O}(M)$.
If we say that, in the convective limit, we expect to converge to the incompressible solution, then it seems reasonable to assume that the entropy field becomes independent of the Mach number $\zeta\sim\mathcal{O}(M^0)$.
If this assumption holds, then the unwanted terms disappear from the limit equation, and the leading order diffusion on the entropy field is an upwinding term with the correct scale, $u$.

\begin{subequations} \label{eq:acoustic_entropy_diffusion_scaling}
Repeating for the acoustic limit, the diffusive terms in the entropy equation are:
\begin{equation}
    u\Gamma\llbracket\phi\rrbracket \sim \mathcal{O}(M^0),
    \quad
    u\llbracket\zeta\rrbracket \sim \mathcal{O}(\zeta)
\end{equation}
and the anti-diffusive terms:
\begin{equation}
    -\Gamma u \mu_p \llbracket\phi\rrbracket \sim \mathcal{O}(M^0),
    \quad
    -\frac{\Gamma u}{\rho a} \mu_u \llbracket u \rrbracket \sim \mathcal{O}(M^0)
\end{equation}
\end{subequations}
In the acoustic limit, the unwanted terms are an order of $M$ larger than in the convective limit, because both $\llbracket\phi\rrbracket$ and $\mu_u$ are an order of $M$ larger.
We do not attempt to estimate the scaling of the entropy field in the acoustic limit here, as this is a complicated topic in and of itself.
For example, we might expect that the viscous entropy generation still be independent of the Mach number, but other phenomena such as entropy noise, combustion and other chemistry may well have a dependence on the Mach number.
We do however explore the coupling of the entropy field to the acoustic subsystem with a numerical example later in the paper.


\subsubsection{Spectral radius of AUSM schemes}
In section ** we found that for schemes which converge to the acoustic limit, the spectral radius (and hence the stability bound) should grow at the same rate as that of the physical flux, $\mathcal{O}(M^{-1})$.
However, for schemes which converge to the convective limit, we estimated that the spectral radius should grow an order of the Mach number faster, $\mathcal{O}(M^{-2})$, due to the contribution of the large diffusion on the pressure field required to enforce a second order pressure variation.

Now we have an approximation of the diffusive flux Jacobian of AUSM schemes (\ref{eq:ausm_diffusion_symmetric}), we can find exact expressions for the eigenvalues of this matrix, and compare how these scale if we assume the diffusion coefficients have the scales we estimated in the previous section (Table \ref{table:ausm_parameter_scaling}).
The exact expressions have been calculated using the symbolic manipulation package Sympy ** (the code for this is included in the supplementary material).
There are two eigenvalues $\lambda_{0,1}$ which are exactly equal to the convective velocity $u$, identically to the physical flux Jacobian.
The corresponding eigenvectors $\mathcal{R}_{0,1}$ are the vorticity and entropy fields:
\begin{equation} \label{eq:linear_eigenvalues_vectors}
    \lambda_{0,1} = u,
    \quad
    \mathcal{R}_0 = 
    \begin{matrix}
    \begin{pmatrix}
    0 \\ 0 \\ 1 \\ 0
    \end{pmatrix}
    \end{matrix},
    \quad
    \mathcal{R}_1 = 
    \begin{matrix}
    \begin{pmatrix}
    0 \\ 0 \\ 0 \\ 1
    \end{pmatrix}
    \end{matrix},
\end{equation}
The expressions for the remaining two eigenvalue/eigenvector pairs, which relate to the acoustic subsystem, are much more complex and unwieldy, so are not included in the main text - the interested reader can refer to Appendix ** for the eigenvalues, and the supplementary material for the eigenvectors.
Instead, by using the scaling requirements in Table \ref{table:ausm_parameter_scaling}, we give leading order estimations to the the largest eigenvalues at the convective and acoustic limits.
At the convective limit we have:
\begin{equation} \label{eq:convective_spectral_radius}
\begin{split}
    \lambda^c_4 & \approx \frac{( \rho a^2 \nu_p + \mathcal{O}(M^{0}) ) + \sqrt{\rho^2 a^4 \nu_p^2 + \mathcal{O}(M^{-2})}}{2} \\
    \lambda^c_4 & \approx \frac{\rho a^2 \nu_p}{2} \\
    \lambda^c_4 & \sim \mathcal{O}(M^{-2})
\end{split}
\end{equation}
This confirms our estimate that AUSM schemes which converge to the convective limit as $M\to0$ have a spectral radius which grows severely as $\mathcal{O}(M^{-2})$.
Previous works in the literature ** have reported instabilities at very low Mach number ($M<0.1$) when using AUSM$^+$-up with explicit schemes.
AUSM$^+$-up was designed for the convective limit, and, as we will show later, the diffusion coefficients have the scaling we found in Table \ref{table:ausm_parameter_scaling}.
The 'fixes' used to alleviate this instability all reduce the value of $\nu_p$ (usually with a cut-off Mach number), which would imply that the instabilities were a result of using a timestep size according to the physical spectral radius, not the one in (\ref{eq:convective_spectral_radius}).
Because the scaling (\ref{eq:convective_spectral_radius}) comes from the requirements on the artificial diffusion, we suggest that it is not a deficiency of the scheme per-se, but rather the necessary price for achieving accurate solutions at the convective limit.
\textit{It's known that implicit schemes are needed for time-accurate preconditioned Roe schemes (convective limit). This shows the same is true for convective limit AUSM schemes. Possible heuristic is that the requirement that the pressure react "instantaneously" to the divergence means some information must travel faster than any physical wave. Incompressible schemes solve the pressure poisson implicity, filtered low mach schemes normally solve some implicit equation for the pressure, why should density based scheme be any different?}

The leading order expression for the largest eigenvalue at the acoustic limit is:
\begin{equation}
\begin{split}
    \lambda^a_4 & \approx \frac{( \mu_u + \mathcal{O}(M^{0}) ) + \sqrt{ (\rho^2 a^2 \nu_p - \mu_u)^2 + \mathcal{O}(M^{-1})}}{2\rho} \\
    \lambda^a_4 & \approx \frac{\rho a^2 \nu_p}{2} \\
    \lambda^a_4 & \sim \mathcal{O}(M^{-1})
\end{split}
\end{equation}
Now the spectral radius scales at the same rate as the physical one, and the stability bound should be well estimated with the usual estimates.
It is interesting that, although $\nu_p$ is asymptotically the smallest parameter in the acoustic limit - 2 orders of $M$ smaller than $\mu_u$ - the leading order approximation of the spectral radius still simplifies down to only contain this parameter.
It is also identical to the leading order approximation at the convective limit, which could be useful as a simple estimate for the spectral radius in a practical CFD code.

\textit{Reference to stability restriction for AUSM+up: Matsuyama, channel flow. HR-SLAU2 papers, 2D shear layer roll up. Iampietro, Daude, Galon, "A low-diffusion self-adaptive flux-vector splitting approach for compressible flows". Chen, Yan, Lin, 2018 - An improved entropy-consistent Euler flux in low Mach number.}

==> sections/ausm_numerical_examples.tex <==
numerical examples
\begin{itemize}
    \item D'Alembert's paradox (canonical convective test)
    \begin{itemize}
        \item drag
        \item Non-dimensional pressure fluctuations
        \item explain influence of pressure extrapolation to wall, run all fluxes with same wall treatment for fair comparison
    \end{itemize}
    \item 1D soundwave (canonical acoustic test)
    \begin{itemize}
        \item show acoustic fluxes all work ok, convective don't
        \item see if restoring the proper scale to $\mu_u$ in the acoustic limit affects the solution.
    \end{itemize}
    \item NACA 0015 airfoil at low Mach
    \begin{itemize}
        \item this case previously shown to produce pressure decoupling with SLAU
        \item SLAU-WS fixed this with in a very ad-hoc manner
        \item show you only need to restore the proper scale to $\mu_p$ to fix this
    \end{itemize}
    \item Low mach 1D shock tube
    \begin{itemize}
        \item very low speed (M=0.0001) contact discontinuity
        \item SLAU and AUSM+up' shown unstable (both have vanishing velocity diffusion as $M\to0$
        \item show can be fixed by restoring velocity diffusion. AUSM+u'p' already does this, SLAU-WS does this in very ad-hoc fashion (show how to do properly for SLAU)
    \end{itemize}
    \item circular cylinder
    \begin{itemize}
        \item inviscid
        \begin{itemize}
            \item Convective scheme is good solution but poor (explicit) convergence
            \item Acoustic scheme is bad
            \item Blended scheme allows small checkerboard but better (explicit) convergence
        \end{itemize}
        \item shedding (Re=150), JFM2002
        \begin{itemize}
            \item Convective scheme has vortex street but no acoustics
            \item Acoustic scheme damps shedding (but maybe has farfield acoustics?)
            \item Blended scheme allows shedding and acoustics (but maybe a bit unstable at v low Mach?)
        \end{itemize}
    \end{itemize}
    \item soundwave through linear fields at acoustic limit: a) entropy bump and b) gresho vortex
    \begin{itemize}
        \item show erroneous diffusion on entropy, but not for vorticity
        \item are there any classic combustion-y test cases we could use to show what effect this actually has on cases of interest?
    \end{itemize}
\end{itemize}

\subsection{1D test cases}
\graphicspath{{./figures/OneD/}}

\subsubsection{Isolated soundwave}
\textit{1) confirm that convective fluxes are unsuitable for acoustic simulations. 2) show acoustic fluxes have excellent resolution with unlimited reconstructions, and that restoring the velocity diffusion only minorly degrades the solutions. 3) show that using fluxes with vanishing velocity diffusion with limiters produces oscillatory solutions, but that these oscillations are removed by restoring the velocity diffusion. \textcolor{red}{This section probably too verbose, try be more curt.}}\\
The first test case we show is an isolated, isentropic, sinusoidal sound-wave in a periodic domain at various Mach numbers.
This test will show the ability (or lack thereof) of a scheme to resolve acoustic waves at low Mach number.
Shima and Kitamura ** previously estimated that SLAU is able to resolve sound-waves without visible decay if at least 40ppw (points per wavelength) are used.
We simulate a marginally resolved wave with 32ppw here, as this results in enough diffusion that the accuracy of different fluxes can be differentiated with the naked eye.
All cases are run for 2048 timesteps with a CFL of 0.5, equivalent to the soundwave travelling 16 wavelengths.
For fluxes with acoustic scaling, a 3 stage, 3rd order SSP explicit Runge-Kutta scheme with a CFL bound of 1 is used **, whereas for fluxes with convective scaling, dual-timestepping with the 2nd order implicit trapezium rule is used due to the restrictive CFL limit we proved in section **.

\begin{figure}[t]
    \centering
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{../place_holder.jpg}
    \caption{}
    \label{fig:soundwave_convective_fluxes}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{../place_holder.jpg}
    \caption{}
    \label{fig:soundwave_acoustic_fluxes}
\end{subfigure}
    \caption{Isolated sinusoidal soundwave at Mach numbers of $10^{-2}$ and $10^{-4}$ with various AUSM fluxes. \ref{fig:soundwave_convective_fluxes} shows fluxes which converge to the convective limit, and \ref{fig:soundwave_acoustic_fluxes} shows fluxes which converge to the acoustic limit.}
    \label{fig:soundwave_unlim_fluxes}
\end{figure}

First, we show the results for AUSM$^+$-up and LDFSS2001.
These are well known to be unsuitable for acoustic simulations, as we confirmed in section ** when we showed that the diffusion of these fluxes converges to the convective limit.
However, we include them here for completeness, to show the drastic differences which are possible between schemes designed for the convective and acoustic limits.
Figure \ref{fig:soundwave_convective_fluxes} shows that after 16 periods these fluxes have completely dissipated the sound-wave, and that it only takes ** periods for the wave amplitude to be halved compared to the initial conditions, confirming the unsuitability of these fluxes for acoustic simulations.

The results for the fluxes that are suitable for the acoustic limit are shown in figure \ref{fig:soundwave_acoustic_fluxes} at Mach numbers of $10^{-2}$ and $10^{-4}$, using an unlimited third order reconstruction.
All these fluxes resolve the sound-wave with very little diffusion, in contrast to those in figure \ref{fig:soundwave_convective_fluxes}.
We also ran Mach numbers down to $10^{-12}$, but the results were indistinguishable from those at $10^{-4}$ so are not shown.
We showed in section ** that SLAU, AUSM$^+$-up' and AUSM-M all have vanishing diffusion on the velocity field as $M\to0$, whereas the velocity in SLAU-u' and AUSM$^+$-u'p' remains well-balanced on all fields.
Unsurprisingly, the two fluxes with non-vanishing diffusion produce solutions which are slightly damped compared to those with vanishing diffusion - the difference in peak velocity between SLAU and SLAU-u' is 3.2\% at $M=10^{-2}$ and 3.3\% at $M=10^{-4}$.
What is perhaps surprising is just how little the solution is affected by the restoration of diffusion on the velocity field, considering that at $M=10^{-4}$, the velocity diffusion term in the interface pressure is $10^4$ times larger in SLAU-u' than in SLAU.

As the solution is smooth, the results shown so far all used an unlimited third order reconstruction.
However, even at low Mach number these fluxes may also be used with limiters if sharp enough gradients are present in the solution (for example in LES, where there is substantial energy at the grid scale).
The results for SLAU and SLAU-u' using Cada's third order limiter ** at Mach numbers from $10^{-1}$ to $10^{-6}$ are shown in figures \ref{fig:soundwave_slau_ca_cada3} and \ref{fig:soundwave_slau_aa_cada3} respectively.
The solutions using SLAU show oscillations in the velocity from a Mach number of $M^{-2}$ and below, although the solution remains stable and somewhat recognisable.
In contrast, the solutions using SLAU-u' are monotone but, compared to figure \ref{fig:soundwave_unlim_fluxes} there is a noticeable flattening of the sin wave, although Mach independence is achieved at the same rate (below $M=10^{-2}$).
For comparison, figure \ref{fig:soundwave_slau_m1e-4} shows results at $M=10^{-4}$ for SLAU and SLAU-u', with unlimited and limited 3rd order reconstructions.
It can be seen that the unlimited SLAU solution has the least diffusion, closely followed by unlimited SLAU-u' solution (3.3\% reduction in peak value), then the limited SLAU-u' solution (18.7\% reduction in peak value).
The limited SLAU solution has oscillations, although the damping is comparable to the limited SLAU-u' solution, and the phase is still mostly accurate.
As the velocity oscillations in the SLAU solutions are not present in the pressure field (not shown), and are removed when the velocity diffusion is restored in SLAU-u', we suspect they are a result of the vanishing diffusion on the velocity field, although we have so far found no satisfactory explanation as to why they only appear in solutions using limited reconstructions.
Second order reconstructions were also tested using a central gradient estimation for the unlimited solutions, and a variaty of methods for the limited solutions, including Minmod, Superbee, Van Albada and Monotonized Central.
Qualitatively the second order results agree with the third order results across the board, so are not shown. The only noteable difference was that the solutions with SLAU and 2nd order limiters were slightly more robust to the oscillations seen in figure \ref{fig:soundwave_slau_ca_cada3}, only appearing at $M=10^{-3}$ and below.

\begin{figure}[t]
    \centering
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{OneD_soundwave_slau_ca_unlim3.png}
    \caption{}
    \label{fig:soundwave_slau_ca_unlim3}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{OneD_soundwave_slau_aa_unlim3.png}
    \caption{}
    \label{fig:soundwave_slau_aa_unlim3}
\end{subfigure}
    \caption{Isolated sinusoidal sound-wave at various Mach numbers, calculated with an unlimited 3rd order reconstruction. SLAU has vanishing diffusion on the velocity field as $M\to0$, whereas the diffusion in SLAU-u' remains well balanced.}
    \label{fig:soundwave_slau_unlim}
\end{figure}

\begin{figure}[t]
    \centering
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{OneD_soundwave_slau_ca_cada3.png}
    \caption{}
    \label{fig:soundwave_slau_ca_cada3}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{OneD_soundwave_slau_aa_cada3.png}
    \caption{}
    \label{fig:soundwave_slau_aa_cada3}
\end{subfigure}
    \caption{Isolated sinusoidal sound-wave at various Mach numbers, calculated with Cada's 3rd order limiter **. SLAU has vanishing diffusion on the velocity field as $M\to0$, whereas the diffusion in SLAU-u' remains well balanced.}
    \label{fig:soundwave_slau_cada3}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{OneD_soundwave_slau_m1e-4.png}
    \caption{Isolated sinusoidal soundwave at a Mach number of $10^{-4}$ with various schemes. SLAU has vanishing diffusion on the velocity field as $M\to0$, whereas the diffusion in SLAU-u' remains well balanced. For the unlimited solutions, the peak value for SLAU-u' is 3.3\% less than the peak value for SLAU.}
    \label{fig:soundwave_slau_m1e-4}
\end{figure}

\subsubsection{Low Mach number shocktube}
\textit{1) reproduce Sachdev et al's result that AUSM+up' produces oscillations around the low Mach contact, which are removed by AUSM+u'p'. 2) link this to our result that AUSM+up' has vanishing diffusion on the velocity field, but that AUSM+u'p' restores this diffusion. 3) show comparable results for SLAU and SLAU-u' (which scale like AUSM+up' and AUSM+u'p' respectively).}\\
This test case was introduced by Sachdev et al **, as a particularly stringent test for fluxes in the acoustic low Mach number regime.
It is a shocktube problem with a very small pressure difference, and the solution consists of two very weak shockwaves travelling in either direction, and an almost stationary contact discontinuity moving at a Mach number of $10^{-4}$.
Sachdev et al found that using AUSM$^+$-up' produced oscillations in the velocity and pressure, as seen in figure \ref{fig:shocktube_ausm}, even though they had designed it for the acoustic regime.
If the initial pressure difference is increased, the Mach number is also increased, and the oscillations are reduced, until they are barely visible at $M=0.1$ **.
In addition, Sachdev et al propose a solution to remove the oscillations completely at all Mach numbers, by using the unsteady Mach number parameter in the calculation of the velocity diffusion in the interface pressure (AUSM$^+$-u'p').
It can be seen from figure \ref{fig:shocktube_ausm} that AUSM$^+$-u'p' produces a monotone solution, albeit with slightly more smearing on the shocks.
We showed earlier that the AUSM$^+$-up' flux has vanishing diffusion on the velocity field as $M\to0$, whereas AUSM$^+$-u'p' has balanced diffusion that remains in the low Mach limit.
We believe that this provides a physical justification both for increasing the velocity diffusion on the interface pressure, and for why this results in a stable scheme for this test case.

\begin{figure}[t]
    \centering
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{OneD_shocktube_M00001_ausm.png}
    \caption{}
    \label{fig:shocktube_ausm}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{OneD_shocktube_M00001_slau.png}
    \caption{}
    \label{fig:shocktube_slau}
\end{subfigure}
    \caption{Weak shock tube flow with a contact discontinuity travelling at $M=0.0001$. SLAU and AUSM$^+$-up' have vanishing diffusion on the velocity field as $M\to0$, whereas the diffusion in SLAU-u' and AUSM$^+$-u'p' remains well balanced.}
    \label{fig:shocktube}
\end{figure}

SLAU was also found to suffer from this instability, shown in figure \ref{fig:shocktube_slau}.
As described in section **, a rather ad-hoc solution was proposed by Shima 2013 ** to rectify both this instability and the checkerboarding at the convective limit.
This solution prevents the velocity diffusion from dropping below a certain cut-off, and uses a pressure-wiggle sensor to locally switch the pressure flux to the convective scale.
Here we propose a more physically motivated solution, by modifying the velocity diffusion in the interface pressure of SLAU in the same manner as AUSM$^+$-u'p', thus resulting in a well-balanced scheme.
The coefficient $M$ in the velocity diffusion equation ** is instead calculated using the unsteady parameter **, so becomes equal to 1 at the acoustic limit.
We call this scheme SLAU-u', and it can be seen in figure \ref{fig:shocktube_slau} that it produces no oscillations for the low Mach number shock tube, and suffers from a much smaller increase in the smearing of the shocks compared to AUSM$^+$-u'p'.

\subsubsection{Interaction of acoustic waves with linear fields}
\textit{1D gaussian soundwave passing through gaussian vorticity / entropy waves. Should show zero modification of vorticity wave before/after but some modification of entropy wave before/after due to negative diffusion terms. Effect will be greater for -u' fluxes as $\mu_u$ is order of M larger.}

\subsection{2D test cases}
